EDO-Net: Learning Elastic Properties of Deformable Objects from Graph Dynamics

We study the problem of learning graph dynamics of deformable objects that generalizes to unknown physical properties. Our key insight is to leverage a latent representation of elastic physical properties of cloth-like deformable objects that can be extracted, for example, from a pulling interaction. In this paper we propose EDO-Net (Elastic Deformable Object - Net), a model of graph dynamics trained on a large variety of samples with different elastic properties that does not rely on ground-truth labels of the properties. EDO-Net jointly learns an adaptation module, and a forward-dynamics module. The former is responsible for extracting a latent representation of the physical properties of the object, while the latter leverages the latent representation to predict future states of cloth-like objects represented as graphs. We evaluate EDO-Net both in simulation and real world, assessing its capabilities of: 1) generalizing to unknown physical properties, 2) transferring the learned representation to new downstream tasks.

==> sections/old/01_Introduction.tex <==
\section{Introduction}

{\color{teal}
There are 3 main components (ordered in importance): i) Learning a representation that encodes the properties given an exploratory action. ii) Conditioning GNN on this representations and representing the cloth with a graph. iii) having a self supervised end-to-end model that first does an exploratory action and then the task in order to predict roolout of graphs given forces as actions. {\color{red}MW: please check if that's correct.}\\

bullet-points to extend on (introduction)
\begin{itemize}
    \item Focus on the example of manipulating (deformable) object that have the same observable properties (shape, size, texture) but different  unobservable properties (mass, elasticity, hardness). If you want to invoke humans take an example and explain how we do a "system identification" step first (we humans do it while we do the task but that's alright). That system identification then allows to adjust the model and perform the task more accurately. (an example could be throwing the different weighted ball or the bed sheet stretching)
    \item Now we motivate why the learning is the best: Can start with the downsides of analytical models and how many hidden propertys could be important for diffretn tasks etc. therfoew we do this "inuitve physics thing" where we learn the representation.
    \item Now the graph is motivated as a representation and then put togheter in the model where we hava an exploratory action to be able to learn the representation and at the same time! learn the task for diffrent samples (diffrent unobservabla properties) in a self supervised end-to-end fashion (this is the rough overview of the mAnaethod)
    \item as a last point highlight the explicit contributions!
    \item we need a meaningfull page 1 fig here as well
    
\end{itemize}
}

% Motivation

Manipulation of deformable objects represents a fundamental skill relevant for tasks such as folding clothes, domestic chores, dressing or bagging groceries~\cite{miller2012geometric, erickson2018deep,canal2019adapting,seita2021learning}. These real world environments are subject to constant changes and perturbations which influence the decision and actions that humans take when interacting with the environment. When the factors of variation of the environment come from the variety of real world deformable objects, an intelligent behavior must account for the different physical properties the objects might have, which influence the dynamics of the interaction \cite{wang2020swingbot}. In these situations, humans have the capability of successfully interact with a new object without the exact knowledge of its physical properties. This can be achieved by leveraging spatial and temporal observations of the environment to adapt their model of the world, which is a compress representation of the environment describing concepts and relationships of the dynamics of the environment \cite{michotte2017perception,ha2018world}. However, teaching robots to generalize their manipulation skills to a wide range of different deformable objects and reasoning about their physical properties has been an highly challenging problem in real world robotic applications~\cite{chi2022iterative}.


% Problems
% State representation of objects with infinite degrees of freedom
% Unkown physical parameter
% No labels for them 
The complexity of learning deformable objects models that generalize to unseen objects arises from two key factors: the state of deformable objects is high dimensional and has no direct representation, whilst  the interaction dynamics are often non-linear and influenced by numerous  physical properties that are hard to estimate and model.
 The first problem can be addressed by representing the state of the deformable object as a graph, which can be extracted from high dimensional observations such as point clouds~\cite{weng2021graph, lin2022learning, ma2021learning}. Graphs represent a powerful tools to describe complex systems and interaction-dynamics, and recent advances in \ac{gnn} research have shown astonishing results in learning complex physics systems involving rigid solids and deformable objects interacting with one another~\cite{sanchez2020learning,pfaff2020learning,sanchez2018graph}. However, in order to model a wide range of interaction dynamics, \ac{gnn}s require information of the physical properties characterizing the system, which might not be easily accessible as previously mentioned. A field of research also known as \emph{intuitive physics} which to address this challenge by learning predictive models with embedded knowledge about physical properties of objects, where the knowledge is obtained by distilling past experiences and interaction observations~\cite{wu2015galileo, mccloskey1983intuitive}. This framework demonstrated that predictive models of multiple dynamics interactions allow to learn a latent representation of the physical properties of the environment without explicit supervision, releasing the need of ground truth annotations of the physical properties of the environments~\cite{finn2017deep, xu2019densephysnet}. Dynamic interactions such as pushing, poking or swinging have been extensively explored in rigid objects literature, but very little work has been done for deformable objects due to the challenges of deformable objects manipulations~\cite{zhu2021challenges, wang2020swingbot, agrawal2016learning}. Nonetheless, recent advances of data-driven techniques for deformable object manipulation suggest that interactions such as flinging or pulling might be relevant to learn an intuitive physics model of deformable objects ~\cite{ha2022flingbot}[resubmission].

% The second problem instead is usually solved with intuitive physics, which does not require to precisely specify the object parameters by learning a latent representation of them. Learning this representation supervisedly however requires labels that are not easily accessible. Research from rigid objects has hovever shown that sel-f supervised losses can help.

%Approaches that try to avoid these problems achieve that through image-based model free learning, which has the downsides of being inefficient especially when multiple tasks are involved~\cite{yan2020learning}. 
% {\comment insert some more related work like intuitive physics, learning latent representation of physical properties and learning graph dynamics of DO. Maybe order inverted}
%Therefore, finding a suitable deformable object state representation aware of the different dynamics that these might exhibit plays a fundamental role in robotics tasks were being aware of the physical attributes of the objects is relevant for the success of the task. Examples are .... Zakory papers ...

%..., many works focused on a method known as intuitive physics \cite{wu2015galileo, agrawal2016learning} which goal is of learning objects physical parameters through learning based approaches and interactions. Knowing a priori what are the physical parameters to be learned and having access to their ground truth are not always a valid assumptions. A common solution to this challenge is to obtain an indirect estimation by learning a feature embedding in a self supervised way \cite{finn2017deep, zeng2020tossingbot, wang2020swingbot}. All of these methods have been shown to work for rigid object, while very little work address the same problem for deformable objects.




%these objects are however presented with many new challenges, most notably the large object configuration spaces, the difficulty of accurate object behaviour modelling, and the large change in the configuration resulting from manipulation attempts.
%One approach employed explicit modelling of cloth deformation in simulation and then attempted to find an optimal trajectory based on the model {\comment cite}. However, those models tend to be very sensitive to the deformation parameters of the objects (stiffness, shear resistance, friction) and therefore do not generalise well to unseen objects or environments or more complex properties of real world objects. (this concept can be in some ways translated to the differentiable simulators)

% Method
We study the problem of learning graph dynamics of deformable objects that generalize to objects with unknown physical properties by leveraging a latent representation of its physical properties, which can be easily adapted to novel object's properties after few interactions. In particular, we focus on elastic physical properties of deformable objects which we explore through a pulling interaction. To enable generalization to unseen elastic properties, we propose a novel method trained on a large variety of elastic properties to jointly learn an adaptive module that extracts a latent representation of physical attributes of deformable objects  and a forward dynamics module to predict future states of the deformable object, which we represent as a graph. 

% to encode a latent representation of physical attributes of deformable objects from high-dimensional observations and to predict future states of the deformable object, which we represent as a graph. 
{\comment finish to describe the method here}
We define an EA to collect observations to learn an adaptation module which updates its representation of a prior belief of the object physical properties with few interaction observations. The define the implicit representation of the world
We learn a graph dynamics model conditioned on this latent representation
We learn both the adaptation and the forward dynamics module through a self-supervised loss without explicit knowledge of the physical parameters of the environment
{\comment focus on the adaptation and the implicit representation}


% Evaluation
We evaluate our approach in both in simulated and real world environments {\comment goal of this week}, where a dual arm robotic manipulator interacts with deformable objects with physical properties never encountered during training. In our experiments, we show that our proposed model is capable to accurately predict the interactions dynamics of a objects with unknown physical properties adapting its internal representation of the physical properties of the object after few observation collected during an exploration phase of the object dynamics. Moreover, we highlight the quality of the learned representation of the physical properties by using it to regress the underlying physical properties of the environment, confirming that our framework can enable the model to learn a latent representation of the physical properties of the object without explicit supervision.
%in particular, we test the generalization capability of our model to predict the dynamic interactions of unseen deformable object. 

% Summary of contribution
In summary, our contributions are:
\begin{itemize}
    \item We propose a model to learn a latent representation of deformable objects physical properties without explicit supervision, alleviating the need of accurately defining the physical properties involved and the need of their ground-truth labels.
    \item We propose a method to explicitly train a forward graph dynamics model of deformable objects to adapt to newly encountered objects with few observations collected through a pulling interaction.
    \item We carry extensive evaluations, both in simulated and real world environments,  of the quality of the latent representation of the physical properties of the deformable objects and the improved performance of our adaptive model to generalize to unseen objects  
\end{itemize}
%Our main contribution is to propose a graph dynamics model that can use few interaction observations to quickly adapt its prior knowledge about the physical properties characterizing the environment and improve future predictions. We propose to learn a latent representation of deformable objects physical properties in a self-supervised fashion by means of a forward dynamics graph model, without the need of explicitly define the physical properties involved and the need of ground-truth labels.We propose a model to explicitly train a forward graph dynamics model to adapt to newly encountered deformable objects after few interactions. We carry extensive evaluations both in simulated and real world environments of the quality of the latent representation of the physical properties of the deformable objects and the improved performance of our adaptive model to generalize to unseen objects  


==> sections/old/01_IntroductionOLD.tex <==
\section{Introduction}

% Motivation
Human capability of manipulating deformable objects is a challenging skill to be taught to robots. Part of this complexity comes from infinite of freedom that these  object have, making unsuitable most of the solution found for rigid objects. Graph representations of deformable object have recently gained popularity due to their low dimensional state space and their capability of modeling complex physics by modeling interactions among particles CITE BATTAGLIA. Most of the times these approaches require to know a priori the parameters characterizing the underlying physics of the object. In real wold scenario however, the assumption of knowing precisely these parameters most of the times does not hold.  


% Research question
Deformable object such as clothes can exhibit a wide range of different dynamics. Depending on the textile material and its construction techniques, the variety of elastic behavior can drastically change and it has to be taken into account in decision processes that involve these dynamics CITE IROS21. 
In order to leverage deformable object properties that are unobservable in static scenario such as elasticity of textiles, robots need to learn how to exploit manipulation strategies in their environment and to observe the outcome of their actions to gain knowledge about the tools they are interacting with.

.. challenges imposed by deformable objects arise from their complex dynamics that are influenced by numerous hard-to-estimate factors such as non-linear anisotropic stiffness, bending factor, density distribution and so on. . Recently, an interest in developing manipulation strategies with high precision requirements increased the interest on methods capable to leverage the variety of behaviors that deformable objects my exhibit due to their physical parameters \cite{chi2022iterative} {\comment another paper that does something like this one for deformable objects?}. But still no work focused the attention on learning an implicit representation of parameters such as elasticity and bending than can adapt to unseen textiles.
...


% Related work
When the mathematical model is known, the definition of the variable involved in the process is straightforward and classical techniques of parameter estimation can be used. The use of complex analytical models, however, comes with the cost of computational complexity of solving and/or optimizing non linear equations. In real world robotic applications, the accuracy of the model is often traded with fast computations to allow online application of the strategies developed CITE HANG SURVEY. When making this trade off, a challenge that arises with deformable objects in to not lose the capabilities of modeling complex and non linear behaviors while keeping the analytical model simple CITE SOME PAPER FROM EC. Data-driven approaches such as neural networks offer a possible solution.
...
To alleviate the need of accurate analytical models, many works focused on a method known as intuitive physics \cite{wu2015galileo, agrawal2016learning} which goal is of learning objects physical parameters through learning based approaches and interactions. Knowing a priori what are the physical parameters to be learned and having access to their ground truth are not always a valid assumptions. A common solution to this challenge is to obtain an indirect estimation by learning a feature embedding in a self supervised way \cite{finn2017deep, zeng2020tossingbot, wang2020swingbot}. All of these methods have been deployed on rigid object, while very little work address the problem of learning parameters of deformable objects due to their complexity.

...missing some related work on people estimating properties and adaptation techniques...

% Contributions
This paper addresses the problem of generalizing goal-conditioned deformable object manipulation to objects with unknown physical (elastic) properties of textiles.
In this work we propose a framework to learn to leverage different elastic properties of textile after few interactions with an unseen objects. We show how with few pulling actions, the robot is capable to tune its prediction for the specific sample he is interacting with. 
%Moreover, we analyse the dimensionality of the problem showing that a structured anisotropy can be taken into account in the specific case of textiles to exploit their anisotropic behavior
{\comment
The contributions are:
\begin{itemize}
    \item a robotic manipulation approach to learn a low-dimensional embedding of textiles physical features from multimodal observations and active exploratory actions
    \item analysis of the correlation between types of observations and level of anisotropy complexity that can be learned?
\end{itemize}
}


The capability of updating these features is of fundamental importance to leverage the variety of physical properties that different deformable objects might exhibit. As these properties are often observable in static scenarios, exploration Actions (EA) defining interactions that exploit these physical attributes are needed

==> sections/old/03_ProblemFormulation.tex <==
\section{Problem Formulation}
%{\comment Problem: learning a forward dynamics model that generalizes to unseen properties $k_i$ of the environment (characterized by physical properties of the environment in this case). This problem has to face two main challenges:
% \begin{itemize}
%     \item precise description of $k_i$ requires expert knowledge (high computational expensive computations for complex systems like deformable objects) and does not scale well with the number of factors of variation of the environments.
%     \item models need to be trained to adapt to change of the environments, but obtaining ground truth values to train data-driven models is not easy, especially in the real world. Need to do it self-supervisely.
    
% \end{itemize}
%  }



{\color{teal}
\begin{itemize}
    \item We should specify exactly what we do here, not be to general -> focus on cloth represented as graphs that have different dynamical behavior determined by unobservable properties. This properties can however be observed indirectly when interaction with the cloth.
    \item lets use the definition tag to be more structured and also able to refer to the definition later in the method when we realise it with NNs
    \item Problem formulation is not a method/motivation section stick to the problem that we address: learning a representation z for the unobservable properties  with an exploratory action and learning the task dynamics (graph/state evalution or whatever) more or less what you have in eq 1.
\end{itemize}
}




%In real world robotic applications, robots needs to operate in constantly changing environments. In this work, we focus on studying environments $\mathcal{E}_i \in \mathcal{E}$ that differs depending on two factors: the type of interaction involved during the manipulation process and the dynamics of the deformable object the robot manipulates. In particular, we analyse  a \emph{bendaging} ($\mathcal{E}^B$) and \emph{lifting} $\mathcal{E}^L$ scenarios, where in the former the interactions are defined by a robot that pulls a bandage over a human arm, while in the latter the robot interacts with an heavy rigid object by lifting it by means of a deformable object. 
In real-world robotic applications, robots need to operate in a constantly changing environment. In this work, we focus on studying environments $\mathcal{E}_i \in \mathcal{E}$ where  the variations $i$ are characterized by different values of the elastic physical parameters describing deformable objects. These physical parameters influence the dynamics of the manipulation, therefore robots need to be aware that different objects might exhibit highly different dynamics in order to manipulate them and possibly predict the outcome of their control actions. We refer to a deformable object characterizing the variation $\mathcal{E}_i$ of  $\mathcal{E}$ as a task $\mathcal{T}_i \in \mathcal{T}$, where $\mathcal{T}$ is the set of all possible deformable object that the robot might encounter in $\mathcal{E}$.

The dynamics of each deformable object $\mathcal{T}_i$ are described by temporal differential equations often \emph{unknown} to the robot, and depends on the physical properties  $k_i \in K$  of the deformable objects where $K$ represents the set of physical properties that characterize the dynamics of $\mathcal{T}_i$.  Physical properties $K$ often used in robotic simulators to model deformable objects are the object mass and the elasticity, shear and bending factors~\cite{hou2019review}. However, for real world non-linear dynamics of deformable objects, estimating the values of these factors to precisely define $k_i$ might require tools unavailable to the robot. Recent data-driven methods alleviate this problem via an indirect estimate of these parameters by learning a latent representation $z_i \in \mathbb{R}^{n_z}$ of the physical properties $k_i$ in a self-supervised fashion without the need for labels or precise definition of the physical properties of the dynamical system~\cite{wang2020swingbot, chi2022iterative} (where $n_z$ represents the dimension of the latent representation). As the physical properties  cannot be inferred from static scenes,  the robot needs to firstly interact with newly encountered deformable object through an \ac{ea}~\cite{wang2020swingbot}.  {\comment too verbose?}
In this work we are interested in addressing the problem of jointly learning a forward dynamics model of deformable objects conditioned on a latent representation $z_i$ of the physical parameters describing the object dynamics, and an adaptation strategy that can adapt $z_i$  to newly encountered objects with few observations $O_i$ recorded during  an \ac{ea}.

% The dynamics of each deformable object $\mathcal{T}_i$, are described by temporal differential equations often \emph{unknown} to the robot, and depends on the physical properties  $k_i \in K$  of the deformable objects where $K$ represents the set of physical properties that characterize the dynamics of $\mathcal{T}_i$, such as mass, elasticity, shearing and bending coefficients etc.  While robotic simulators model these properties $K$ using physical models such as mass-spring or FEM~\cite{hou2019review}, in real world scenarios estimating the values of these factors to precisely define $k_i$ is not trivial and might require tools unavailable to the robot. Recent data-driven methods alleviate this problem via an indirect estimate of these parameters by learning a latent representation $z_i$ of the physical properties $k_i$ in a self-supervised fashion without the need for labels or precise definition of the physical properties of the dynamical system~\cite{wang2020swingbot, chi2022iterative}. Since these physical properties affect the dynamics of the deformable object, they cannot be inferred from static scenes, independently on how they are represented (implicitly or explicitly) ({\comment use previously implicitly or explicitly}). Therefore, the robot needs to firstly interact with newly encountered deformable object through an \ac{ea} in order to observe these physical properties~\cite{wang2020swingbot}.
% In this work we are interested in addressing the problem of jointly learning a forward dynamics model of deformable objects conditioned on a latent representation of the physical parameters describing the object dynamics, and an adaptation strategy that can update the latent representation of the physical properties of the model to newly encountered objects with few observations $O_i$ recorded with an \ac{ea}.

% the idea of learning these properties in a self-supervised manner comes from the fact that the ground-truth values of these properties are lacking. If no labels are present, these properties are unobservable from a single observation. One way of obtaining them is measuring the dynamics response of the deformable object to a certain interaction. This is the inspiration for the model, and we rely on techniques commonly used in the textile industry to extract these information from clothing items (stress-strain test)..

%State representations of deformable objects are usually based on geometric discrete representations such as particle or meshes \cite{yin2021modeling}. 
We define the state of $\mathcal{T}_i $ as a graph $G_i = (V_i, E_i)$ with nodes $v_^i \in V_i$ and edges $e_^i \in E_i$. 
The features of the node $v_n^i$ describe the position of the nodes in the 3D Cartesian space, while the features of the edge $e_{ns}^i$ characterizing the interaction among nodes, which in our case we augment with the latent representation $z_i$ of the physical attributes $k_i \in K$. The aim of this work is to learn a graph dynamics model of deformable objects $g_\theta$ conditioned on a latent adaptive representation $z_i$ of the underlying elastic physical properties $k_i$ of the system $\mathcal{T}_i $:
\begin{equation}
    g_\theta(G_i^t , a_i, z_i) = G_i^{t+1}.
    \label{eq:graph_dyn}
\end{equation}
The latent representation $z_i$  can be adapted to new and unseen samples through a learned function $f_\phi$ takes as input  the observations $O_i$ obtained applying the exploratory actions $EA_i$ to $\mathcal{T}_i$, a $z_0$ is a prior belief about the object's physical parameters and maps them into $z_i$:
\begin{equation}
    f_\phi(\mathcal{O}_i, EA_i, z_0) = z_i
    \label{eq:adapt_f}
\end{equation}
where the initialization of $z_0$ is learned along the model's parameters.
 In what follows, we will describe in details the method to implement and train the graph dynamics and adaptation functions, respectively $g_\theta$ and $f_\phi$.
 %This section describes the method to learn a graph dynamics model $g_\theta$ of deformable objects that can adapt to variations $\mathcal{E}^i$ of the environment $\mathcal{E}$ through a learned functions $f_\phi$ maping the observations obtained through an \ac{ea} to a latent representation $z_i$ of the physical properties defining $\matchal{E_i}$. 
We make the assumption that the input state of the forward dynamic model $g_\theta$ is always a static state, meaning that there are no forces applied to the object. This assumption allows us to study the scenario where complete information about the physical properties of the object cannot be retrieved from the input of the forward model, .  


%%%%%%%%%%% OLD VERSION

%In real world applications, the dynamics of deformable objects are described by temporal differential equations often \emph{unknown} to the robot. These dynamics depend on physical properties that cannot be inferred from static scenes. Therefore, in order to observe these physical properties the robots need to execute an \ac{ea}  \cite{wang2020swingbot}. In this work we are interested in addressing the problem of learning task specific dynamics of deformable objects such as textiles that can update the internal representation of the physical properties of newly encountered objects after few interactions. We focus our work on textiles for sake of comprehension, but the same type of reasoning could be transferred to any type of system that can be described as a graph and the interactions among nodes depends on physical properties that varies across different sample. {\comment last sentence can be removed}

% Graph representation for clothes, define the task and the state representations
%Dynamics model of deformable objects are usually based on geometric discrete representations such as particle or meshes \cite{yin2021modeling}. We refer to each textile sample as a task $\mathcal{T}_i \in \mathcal{T}$, where $\mathcal{T}$ is the set of all possible textiles. We define the state of $\mathcal{T}_i $ as a graph $G_i = (\mathcal{V}_i, \mathcal{E}_i)$ with nodes $v_n^i \in \mathcal{V}_i$ and edges $e_{ns}^i \in \mathcal{E}_i$.
% We focus on elasticity and say that properties are encoded in the edges
%The features of the node $v_n^i$ describe the position of the nodes in the 3D Cartesian space, while the features of the edge $e_{ns}^i$ are the representation of the physical attributes $k_i \in K$  characterizing the interaction among nodes where $K$ is the set of all elastic physical properties. Given a textile $\mathcal{T}_i $, relevant physical properties $k_i$ to describe its elastic mechanical behavior are its mass, surface friction, elasticity, shear and bending factors \cite{hou2019review}.  For complex and non-linear dynamics such as the ones of textiles, estimating the precise value $k_i$ is challenging and might require tools unavailable to the robot. Recent methods alleviate this problem via an indirect estimate of these parameters by learning a latent representation in a self-supervised fashion  \cite{wang2020swingbot, chi2022iterative}.



% the way to exploit these properties is through interaction, that for the case of elasticity  is pulling.
 

%The aim of this work is to learn a graph dynamics model of textiles $g_\theta$ conditioned on a latent adaptive representation $z_i$ of the underlying elastic physical properties $k_i$ of the system $\mathcal{T}_i $:
% \begin{equation}
%     g_\theta(G_i^t , a_i, z_i) = G_i^{t+1}
%     \label{eq:graph_dyn}
% \end{equation}
% The latent representation $z_i$  can be adapted to new and unseen samples through a learned function $f_\phi$ that maps the observations $\mathcal{O}_i$ obtained applying the exploratory actions $EA_i$ to a new sample to the object's specific $z_i$:
% \begin{equation}
%     f_\phi(\mathcal{O}_i, EA_i, k_0) = z_i
%     \label{eq:adapt_f}
% \end{equation}
% where $k_0$ is a prior belief {\comment still to be seen if we really want to have a prior belief or not} about the object's parameters.
%  In what follow, we will describe in details the method to implement and train the functions $g_\theta$ and $f_\phi$ {\comment we might find specific names to refer to these two modules, like dynamic module and adaptation module}.

% The method therefore has to define the action that is a specific force perceive, the observaion is the displacement of the object observed through either graphs, images, pointcloud etc... and from there the information about the elastic properties can be extrapolated.

% We model the graph dynamics through the GNN,...
% We assume our observations are.. and the actions are....
% We define k_i as features that are disposed as an adjacency matrix.
% We use the observations to regress K in this way: learned mapping or MAML....
% We use this feature in a dynamic prediction task...


==> sections/old/04_method.tex <==
\begin{figure*}[t!]
  \centering
         \includegraphics[width=0.45\textwidth]{images/method.pdf}
         \includegraphics[width=0.45\textwidth]{images/Predict.png}
        %  \caption{Prediction of SIM mesh.}
    \caption{Scheme of the overall model. The adaption module (red  block) update a prior belief $z_0$ of the latent representation of the physical attributes of the textile $\mathcal{T}_i $ from sequences of observations ($O_t^s$, $O_t^b$) recorded via predefined interactions of the object (\ac{ea}). The forward dynamics module $g_\theta$ leverages on the representation $z_i$ obtained from the adaptation module to compute accurate prediction.}
    \label{fig:dyn_model}
\end{figure*}

\section{Method}

% \begin{figure*}[t!]
%   \centering
%          \includegraphics[width=\textwidth]{images/Full_Model.png}
%         %  \caption{Prediction of SIM mesh.}
%     \caption{Scheme of the overall model. The adaption module (red  block) update a prior belief $z_0$ of the latent representation of the physical attributes of the textile $\mathcal{T}_i $ form sequences of observations ($O_t^s$, $O_t^b$) recorded via predefined interactions of the object (EA$^s$, EA$^b$). The forward dynamics module $g_\theta$ leverages $z_i$ to compute accurate prediction.}
%     \label{fig:dyn_model}
% \end{figure*}

An overall picture of the proposed framework is shown in Fig.~\ref{fig:dyn_model}, where it can be noticed that the method consists of two modules: \textbf{adaptation} and \textbf{graph prediction}. In particular, each time the environment changes by introducing an unseen deformable object $\mathcal{T}_i$ with unknown physical properties, the robot has to adapt his prior belief $z_0$ about the object to obtain latent a representation $z_i$ of its \ac{pp}. To do so, the robot needs to interact with the object through an EA and collect a set of observations $O^{EA^i}$ such that the adaptation module that maps them into $z_i$ via the learned function $f_\phi$.
This latent representation is leveraged by the forward model $g_\theta$ to obtain accurate predictions of the future states of $\mathcal{T}_i$ conditioned on different interaction.
%. i.e. states where no forces are applied to the deformable objects and no information about the physical properties of $\mathcal{T}_i$ can be observed.  %interactions $\mathcal{D}_i = \{G_t^i, G_{t+1}^{i}, a_t\}$ between the robot, the deformable object and the objects present in the environment $\mathcal{E}_i$. The initial state $G_{t}^i$ represents a static state  

%This section describes the method to learn a graph dynamics model $g_\theta$ of deformable objects that can adapt to variations $\mathcal{E}^i$ of the environment $\mathcal{E}$ through a learned functions $f_\phi$ maping the observations obtained through an \ac{ea} to a latent representation $z_i$ of the physical properties defining $\mathcal{E_i}$. 
%These variations manifest as differences among physical properties $k_i\in K$ of the deformable objects, which can be observed in dynamics scenarios. Therefore,   

As our approach is founded on the assumption that we represent the state of  $\mathcal{T}_i $ as a graph $G_i = (V_i, E_i)$, in what follows we will provide the details of the two aforementioned modules assuming that the state $G_t^i$ of the object at time $t$ is directly observable. However, we will drop this assumption in the last paragraph of this section, considering a proxy observation of the ground truth state of the object such as a \ac{pcd}.  Moreover,  we make the assumption that the input state $G_t^i$ of the forward dynamic model $g_\theta$ is always a static state, meaning that there are no forces applied to the object. This assumption allows us to focus our study-case in the scenario where complete information about the physical properties of the object cannot be retrieved from the input of the forward model, highlighting the necessity of leaning $z_i$.  
% how we extract $z_i$ from few interactions and how we model the graph dynamics of deformable object
% {\comment don't like it so much}



\subsection{Exploration Action and Adaptation}
% we define how these properties can be distributed along the textile/cloth: isotropic, structured, fully anisotropic
%{\comment The discussion that follow will be removed while we don't use the anisotropy} Depending on how the elastic properties are distributed in the edges, we can distinguish three type of elastic responses of a textile sample: \emph{isotropic}, \emph{structured anisotropic}, \emph{anisotropic}. The first case corresponds to the scenario where the edge properties are equal for each edge. The structured anisotropy assumes instead that edge properties are grouped with respect to a predefined structure. Usually, for textiles, this structure is defined by warp and weft directions. The fully anisotropic case instead has no clear pattern among the distribution of the edge properties along the path, which concretely can correspond to patches applied to the textiles, sews or anything that could influence the elastic property of an edge. In this work we will focus on \emph{isotropic}  samples. 

%tensile stress and a bending stress like shown in fig. \ref{fig:EA} to exploit respectively the stiffness and bending properties of the objects.
\begin{figure}[h!]
  \centering
         \includegraphics[width=\linewidth]{images/plling.png}
        %  \caption{Prediction of SIM mesh.}
    \caption{Exploration Actions - Pulling to observe graphs and forces }
    \label{fig:EA}
\end{figure}


%For linear elastic models, the observation $\mathcal{O}_i$ of the displacement of $\mathcal{G}_i $ under a specific tensile load is enough to fully characterize the elastic parameters $k_i$ through the Hooke's law.  {\comment might be shortened}
%To observe the physical properties $k_i$ of a deformable object $\mathcal{T}_i$ the robot needs to perform an \ac{ea} and observe the response of the object, which will behave accordingly to $k_i$. 

Industrial evaluations to measure physical attributes of deformable objects rely on mechanical stress tests, where a predefined load is applied on the object and its deformation is observed to infer the physical properties \cite{yousef2018investigating}. We translate this concept into a robotic framework  like shown in Fig.~\ref{fig:EA}, where a two-arms robotic manipulator grasping $\mathcal{T}_i$ from its edges exerts a tension stress on it by pulling the edges along opposite directions similarly to what done in \cite{longhini2021textile}, [resubmission]. During this \textbf{pulling} interaction ($\ac{ea}^i$ ), the robot records a set of observations $\mathcal{D}^{EA^i} = \{O_t^i, \}_{t = 1,...,T}$ where $O_t^i$ consists on the state $G_t^{EA_i}\in \mathbb{R}^{N\times 3}$ of the object, where $N$ is the number of nodes, and the force $F_t^{EA_i}\in \mathbb{R}^{3}$ perceived at time $t$ from the robot sensors. As just few observations are needed to retrieve the physical properties of {\comment would be nice to have an experiment showing this}, we randomly select $n_a$ observations $\mathcal{D}^{A^i} = \{G_a^i, F_a^i\}_{a = 1,...,n_A}$ , and a function $f_\phi$ distills the knowledge contained in the observations to adapt a prior belief $z_0$ about the physical properties. The initialization of the prior belief is learned end-to-end the initialization, but it could be set arbitrarily to any sensible value related to the problem addressed {\comment we might evaluate different initialization of $z_0$ and have an ablation study that evaluates them}.
To implement the adaptation function $f_\phi$ in eq. (\ref{eq:adapt_f}), we process each observation  $\{G_a^i, F_a^i\}_{a = 1,...,n_A}$ by firstly concatenating $F_a^i$ to each node $v^i_n \in V^i$ and by projecting the concatenation in a latent embedding $\{o^i_{a_{v_n}}\}_{v_n \in V^i} \in \mathbb{R}^{n_o}$. To extract graph global features $\{x^i_{a}\}_{a = 1,...,n_A} \in \mathbb{R}^{n_x}$ from $\{o^i_{a_{v_n}}\}_{v_n \in V^i}$, we learn a weighted aggregation function of the nodes through an attention mechanism {\comment cite attention and GAT} such that:

\begin{equation}
    x_a = \Omega  \left(\sum_{v_n\in V^i}  \alpha_n o^i_{a_{v_n}}  \right)
\end{equation}

where $\alpha_n$ is the learned attention weight for the node $n$ and $\Omega: \mathbb{R}^{n_o} \rightarrow \mathbb{R}^{n_x}$ is a projection function implemented as a \ac{mlp}. For details about the implementation of the attention mechanism, we refer the reader to {\comment GAT and attention mechanism}.


%The selected sequence of observations is firstly encoded in a latent vector $\{o_{a}\}_{a=1,...,n_a} \in R^{n_d}$ through a modality specific encoder $E_{\phi}$. The architecture of $E_{\phi}$ consists on {\comment x} \ac{mlp} projecting the nodes $v^i_n \in V$ into a latent embedding $h^i_n \in \mathbb{R}^n_v$, where $n_v$ is the dimension of the embedding. To encode global information about the object, we add an attention layer that projects the $h^i_n \in \mathbb{R}^n_v$ into en embedding of the same size of $z_0$, obtaining the final encoding ${o_{a}}_{a=1,...,n_a} \in R^{n_d}$ by averaging the output of the attention layer across all the nodes. 

The latent representation $z_i \in \mathbb{R}^{n_z}$ is finally obtained by using $\{x^i_{a}\}_{a = 1,...,n_a}$ to recursively adapt the prior belief $z_0$ through a \ac{rnn} parameterized by a weight matrices $W_x \in \mathbb{R}^{n_z\times n_x}$ and  $W_z \in \mathbb{R}^{n_z\times n_z}$, which yields the following update rule:  
\begin{equation}
    z_a =\text{tanh} \left(  W_x x_a^i +  W_z z_{a-1} \right), \; a=1, ..., n_a
\end{equation}
where $z_i \equiv z_{n_a} $.
%The \textbf{bending} interaction (EA$^b$) is meant instead to exploit the bending characteristics of the textile {\comment provide more details}. 
%To evaluate the deformation of the object in response to each EA executed, we record a sequence of $n_o$ observations $O_t^s$ of the state $G_t$ of the object. 




%\subsection{Adaptation Module}
% Goal is to adapt to new samples
%To adapt the forward dynamic model to an unseen textile sample $\mathcal{T}_i $, the latent representation $z_i$ of the object physical properties $k_i$ has to be inferred form the sequences of observations  $O_t^s$ and $O_t^b$ collected via the execution of respectively EA$^s$ and EA$^b$.  
% The observation obtain through EA are firstly encoded, the encoders depend on the modality of the observation. For images  CNN, for graphs GNN (or MLP), and for PCD?
%The architecture of $E_{\phi}$ depends on the modality of the observation, we use a GNN to encode graphs, a CNN to encode images and Pointnet \cite{qi2017pointnet} to encode PCD. 
% Combination of encoding of observation and prior belief of the latent representation of z0 is fed to a network that infer the update of the belief such that ... equation ...

% the optimal initialization of z0 is learned EE (might see whether we have a better way to initialize it)



\subsection{Forward Dynamics Module}


To model the graph dynamics in eq. \ref{eq:graph_dyn} we use a Graph Neural Network (GNN) parameterized by $\theta$ trained to predict state differences $\delta G_i^t$ given the current state $G_i^t$, the action $a_t$ and the latent representation of the object physical properties $z_i$. The actions corresponds to the control inputs of the robotic manipulator, which are interactions applied on a subset of the nodes and can be either force or displacement commands. 

%%%%%%%%%% MULTI HOP EDGES %%%%%%%%%
%The definition of the physical feature embedding $z_i$ draws inspiration from mesh based models describing elastic behaviors like the mass-spring systems. In these frameworks the particles are interconnected with mass-less springs that can be categorized in \cite{hou2019review}: \emph{1-Hop spring} - connect nearest  neighbor describing stiffness and shearing properties, \emph{2-Hops spring} - connect second neighbor along the line describing bending properties. 
% \begin{figure}[h!]
%   \centering
%          \includegraphics[width=\linewidth]{images/Z_format.png}
%         %  \caption{Prediction of SIM mesh.}
%     \caption{Representation of the physical features. The first half of $z_i$ describes stiffness and shearing properties (blue - 1-Hop neighbors), while the second half represents the bending properties (green - 2-Hops neighbors). }
%     \label{fig:featrue_rep}
% \end{figure}


%Fig. \ref{fig:featrue_rep} illustrates how we borrowed this notion to represent and integrate the embedding of physical feature $z_i \in \mathcal{R}^{d_z}$ into the GNN architecture, where $d_z$ represent the dimension of the feature embedding. The first half of  $z_i$ describes the stiffness and bending properties among 1-Hop neighbors ($N^{(1)}$), while the second half relates to bending attributes among  2-Hops neighbors ($N^{(2)}$).
An encoder parameterized with a Multi-Layer Perceptron (MLP) maps the concatenation of nodes and actions $a_t$ into a hidden state $h_n^0 \in \mathbb{R}^{d_n}$. The interactions among nodes are computed via an $M$ step learned message-passing which generates a sequence of updated hidden states with the following update rule:
\begin{equation}
    h_n^m = \Phi\left( \sum_{s\in \mathcal{N}_s} \Psi \left( h_n^{m-1}, h_s^{m-1}, z_i \right)   \right) \quad \forall v_n \in V_i.
\label{eq:prop}
\end{equation}
where the aggregations happen across the neighbors $\mathcal{N}_s$ of the node $s$, while $\Psi $  and $\Phi $ are respectively the learned message and update functions parametrized as MLPs. {\comment missing something higlighting that $z_i$ is considered as edge feature and the parallel computations among neighbors} 
% MULTI HOP COMPUTATION
%The parallel computation of 1 and 2-Hops neighbor allows to learn more complex relationship functions among neighbors such as the bending property \cite{abu2019mixhop} {\comment can we also have an experiment to support this claim?}. The $M$-th hidden state is finally projected in the nodes displacement through a decoder implemented with an MLP. 

\subsection{Self-Supervised Loss}

The overall model can be learned using a dataset of exploratory observations $\mathcal{D}^{EA} = \{\mathcal{D}^{EA^i}\}_ { i \in [1, N_k]} $ and a dataset of interactions $\mathcal{D} = \{\mathcal{D}_i\}_ { i \in [1, N_k]} $,  where  $N_k$ is the number of different textile $\mathcal{T}_i \in \mathcal{T}$. The parameters $\phi$, $\psi$, $\theta$ and the prior belief $z_0$ can be optimized using a supervised loss on the prediction of the state $G_i^{t+1}$ obtained from $g_\theta$ conditioned on $G_t^i, a_t$ and the adapted latent representation $z_i$. The loss function can be defined as follows:
\begin{multline}
    \mathcal{L} (\phi, \psi, \theta, z_0; \mathcal{D}^{EA},\mathcal{D} ) = \\
    =    \mathbb{E}_{\mathcal{T}_i \sim \mathcal{T}} \left[ \mathbb{E}_{\mathcal{D}_i, \mathcal{D}^{EA^i}} \left[ d(G_i^{t+1} - g_{\theta}(G_i^t, a_t, z_i)) \right]\right]\\
    \text{such that} \; z_i = f_\phi ({O_a^i}, z_0)
    \label{eq_loss}
\end{multline}


where  $d$ is a distance measure between the ground truth state of the textile and the model's prediction. In our case, $d$ corresponds to the Mean-Squared Error (MSE). Equation \ref{eq_loss} optimizes the model parameter to learn a forward dynamic function $g_\theta$ which leverages different objects properties $k_i$ through an implicit representation $z_i$, where $z_i$ is obtained from $f_\phi$ few observed interactions with a newly encountered object.

\subsection{Graph extraction from point clouds}

In many real world applications, however, the ground truth graph might be challenging to obtain. Therefore, in this work we evaluate also the performances of proxy observations of the ground truth graph depending on the sensing modality available. In particular, we consider as proxy observations \emph{point-clouds} that are easily accessible from camera sensors.  

To extract the graphs from the observation given as point clouds, we train Pointnet \cite{qi2017pointnet} to output a graph of fixed size, using as ground-truth the states provided by the simulator. We then align the point clouds from the real world to the simulation ones, given the unavailability of graphs in the real world. However, the model is agnostic to the type of processing to obtain the graph and other graph extraction techniques as the ones in \cite{ma2021learning, lin2022learning} can also be used.

To extract the graphs from the observations given as point clouds, we use {\comment (fill in with Michael's method)}, to output a graph of size {\comment x}, both for simulation and real world data. { \comment (Don't know if we want to mention the next part...) We decide to fix the size of the graph for easier training and evaluation, but the formulation with \ac{gnn} allows to be agnostic to the size of the graph, giving the possibility of changing the dimensionality of the representation according to the application.}



==> sections/old/05_experiments.tex <==
\section{Experiments}
In this section we want to evaluate both in simulation and in the real world the learned latent representation $z_i$  and the capability of the forward model to generalize over a variety of physical properties of cloth-like deformable objects.
%The experimental evaluation aims at showing the capability of the proposed model to learn how to generalize over a variety of physical properties of deformable objects influencing their dynamics. We evaluate both the performance of the forward dynamics model and the quality of the adaptation module in learning a representation $z_i$ of the physical properties. 
To this aim, we carry the following evaluations:
\begin{enumerate}
    \item We test the performance of the forward dynamics model in a state prediction downstream task over a set of deformable objects $\mathcal{T}_i \sim \mathcal{T}$ with \emph{unseen} elastic physical properties $i$. 
    % \item We qualitatively evaluate the learned representation by visualizing a UMAP projection of the latent space of the learned parameters.
    \item We  examine in simulation how accurately we can decode physical properties from the learned representation by learning a regressor of the ground-truth parameters on top of the learned representation $z_i$.
    \item We quantitatively evaluate both in real world and simulation whether the learned representation encodes information about deformable object physical properties by learning an inverse model conditioned on the learned representation $z_i$ to predict the control action between two consecutive frames.
    \item We carry an ablation study on the influence of the length $T$ of the sequence of observations $O^i$ to encode $z_i$, and on the architectural choices for the overall model. 
    % {(\comment also type of \ac{ea} if we have the time)}.
\end{enumerate}
{\comment I would put the baselines at the beginning of each evaluation section, as they change depending on the experiments we have}

We compare the performance of the forward dynamics module with the following baselines:
\begin{enumerate}
    \item \textbf{Baseline:} $g_\theta$ is trained to predict $\hat{G}_i^{t+1}$ given only the initial state $G_t$ and the action $a_t$, without any conditioning on $z_i$. 
    \item \textbf{Supervised:} $g_\theta$ is trained to predict $\hat{G}_i^{t+1}$ while $f_\phi$ is also trained to predict the ground-truth simulation parameters. 
    % {(\comment enough or do we need to give more details?)}
    \item \textbf{Oracle:} the forward model $g_\theta$ is conditioned on the ground-truth simulation parameters.
\end{enumerate}


\subsection{Simulation Setup}
We implement a simulation environment in Pybullet \cite{coumans2021, erickson2020assistive}, involving two end-effectors of Franka-Emika Panda robots equipped with Force/Torque sensors. 
The \ac{ea} visible in Figure~\ref{fig:contexts} consists in pulling the edges of a square cloth in opposite directions to extract the graph $G_t^{EA^i}$ and force $F_t^{EA^i}$ observations, as introduced in Section~\ref{sec:method_EA} . We define a \textit{bandaging} and a \textit{lifting} interaction between the deformable object manipulated by the robot and an external rigid object (Figure~\ref{fig:tasks}). In particular, in the \textit{bandaging} interaction the robot holds and pull the cloth over a human arm, gradually moving downwards and hence applying an increasing force on the arm. %, where this force is dependent on the chosen physical parameters.
In the \textit{lifting} interaction, instead, a sphere is positioned on the cloth and the robot lifts it up to a certain altitude. These interactions aim at emulating scenarios in which different physical properties of the manipulated object influence the outcome of the robot control actions, where to generate a large variety of physical properties of the cloth we varied both the \textit{stiffness} and \textit{bending} parameters used by the simulator to model the deformable object. %have different effects on its deformation and on the force it exerts on external objects.
An example of the different behaviours that the cloth exhibit is visible in Figure {\comment (ref to figure to show this in both tasks)}
{\comment to be modified to one single dataset}
We collect 2 datasets in which we vary respectively the stiffness and the bending parameters. The parameters vary in the range $[10, 45]$ for elasticity, with a step of $3.0$, and $[0.01,5.01]$ for bending, with a step of $0.5$. The environment is scaled by a factor of $5$ to avoid instability of the clothing object in the simulation.

% {\comment it could be useful to have a figure showing the variation of forces due to the different parameters}

\begin{figure}[t!]
  \centering
         \includegraphics[width=\linewidth]{images/contexts.png}
        %  \caption{Prediction of SIM mesh.}
    \caption{The pulling EA collected varying the stiffness and bending parameters.}
    \label{fig:contexts}
\end{figure}

\begin{figure}[t!]
  \centering
         \includegraphics[width=\linewidth]{images/tasks.png}
        %  \caption{Prediction of SIM mesh.}
    \caption{On the left, the \textit{object lifting} task used to assess the capability of the model in accounting for different bending parameters. On the right, the \textit{arm wrapping} task, used for the stiffness parameters.}
    \label{fig:tasks}
\end{figure}

\subsection{Network Architecture and Training details}
% adaptation function details: observations encoder and attention module, RNN, dimension of z_i
For each observation $O_t^{EA^i}$, we used an \ac{mlp} with one hidden layer of size $32$ to implement the node encoder of the adaptation module, while the attention layer is implemented as a learned linear projection from the encoded node $o_v\in\mathbb{R}^{32}$ to the attention value $\alpha_v \in \mathbb{R}$. The aggregation of the nodes $z_i^t$ for each temporal observation is processed through an RNN with one hidden state which starts with a prior belief $z_0 \in \mathbb{R}^{32}$ and outputs $z_i \in \mathbb{R}^{32}$ as its last hidden state~\cite{rumelhart1986learning}. We empirically chose the size of  $z_i=32$ as the one with highest performance across all the evaluations, while we learn the initialization of $z_0$ along the networks parameters.
% fowrard model details: nodes encoder, propagation layers (message encoding and aggregation function) plus the number of propagation steps. projection layer.
We implemented the forward dynamics model as a standard message-passing network parallelizing the computation of the $1\-st$ and $2\-nd$ order neighbors~\cite{li2019propagation, abu2019mixhop}. We propagate the information for $M=4$ steps, while we implement the node's encoder, the final linear projection and the message and the aggregation functions as \ac{mlp}s with one hidden layer of size $32$. We use ReLU as non-linearity for all the modules execept the RNN, where we used tanh as activation function.
% Training details, batch size, epochs, lr, optimizer, 

The models are trained for $10k$ epochs and batch size equal to $8$. We used ADAM with learning rate of $0.001$ and weight decay equal to $10^{-5}$~\cite{kingma2014adam}. We split the simulation dataset in train, validation and test dataset, using the validation dataset to select the best performing model during training.  We subsequently test the the model on the test dataset to ensure that the physical parameters of the deformable objects are unseen to the model. In real world, instead, we rely only on training and test set due to the smaller size of the datataset available.
 
% Train, val, test split.
%training dataset for $10k$ epochs, selecting as best model the one achieving higher performance on a validation dataset. We subsequently test on an held-out dataset to ensure that the physical parameters of the deformable objects are unseen during training.

\subsection{Forward module evaluation}
% \subsection{Algorithm experiments}
We evaluate the forward dynamics module in both state prediction and action prediction.
In the state prediction evaluation, the forward dynamics module receives the initial observation of the cloth $G_i^t$ and the control action $a_t$, and is asked to predict the graph at the following time step $G_i^{t+1}$. The performance is the mean square error computed between the graph $G_i^{t+1}$ and the graph predicted by the model $\hat{O}_i^{t+1}$. The pseudo code of the algorithm can be seen in Alg. \ref{alg:eval}, while the results are shown in Table \ref{tab:state_prediction} for both environments. 

% \begin{algorithm}[!ht]
% \DontPrintSemicolon
%   \KwInput{EA$^i$, O$^i$, $a^t$, $G_i^t$}
%   \KwOutput{$\hat{G}_i^{t+1}$}
%   \KwData{Testing set $\mathcal{T}_i \in \mathcal{T}$}
  
%   $z_i = f_\psi ( E_\phi (O^i, EA^i))$\\
%   $\hat{G}_i^{t+1} = g_\theta (G_i^t, a^t, z_i)$ \\
%   $e = \lVert \hat{G}_i^{t+1} - G_i^{t+1} \rVert$ \\
 
% \label{alg:state}
% \caption{State prediction evaluation}
% \end{algorithm}

\begin{table}[!h]
    \centering
    \caption{Comparison with number of adaptation samples =3 }
    \begin{tabular}{lcc}\toprule
         Model & State Error [mm$^2$] &  State Error [mm$^2$]   \\
                &  Bandaging  &    Lifting                      \\
        \toprule
        
         Baseline               &  4.229            \pm \; \;   8.923   & 3.323             \pm \; \;   6.566     \\ %\toprule
         Supervised             &  0.928            \pm \; \;   1.579   & 0.099             \pm \; \;  0.045        \\ %\midrule
         \textbf{Ours}          &  \textbf{0.133}   \pm \; \;   0.168   & \textbf{0.085}    \pm \; \; \textbf{0.058}\\ \bottomrule
         Oracle                 &  0.103            \pm \; \;   0.099   & 0.074           \pm \; \;    0.040        \\ %\midrule
   
    \end{tabular}
    \label{tab:state_prediction}
\end{table}


% \begin{table}[!h]
%     \centering
%     \caption{Comparison with number of adaptation samples = 5 }
%     \begin{tabular}{lcc}\toprule
%          Model & State Error $*10^{-3}$ &  State Error $*10^{-3}$    \\
%                 &  Bandaging  &    Lifting                      \\
%         \toprule
        
%          Baseline               &  -            \pm \; \;   -   &    6.5845         \pm \; \;    12.786    \\ %\toprule
%          Supervised             &  -            \pm \; \;   -   &    0.3211           \pm \; \;  0.6993        \\ %\midrule
%          \textbf{Ours}          &  -              \pm \; \;   -   &   0.1020    \pm\;\; 0.0684 \\ \bottomrule
%          Oracle                 &  -            \pm \; \;   -   &     0.0808      \pm \; \;     0.0399       \\ %\midrule
   
%     \end{tabular}
%     \label{tab:state_prediction}
% \end{table}


In the action prediction evaluation, the model is asked to choose the best control action to perform given a desired target state $G_i^T$ to reach. The procedure is the following: we uniformly sample actions $a_j \in [0, a_{max}]$ and we query the forward model to predict the next state $G_i^j$ for each of the sampled actions. The best action $a^*$ selected is the one for which the error between the predicted state $G_i^*$ and the target state $G_i^T$ is the minimum. The pseudo code of the algorithm can be seen in Alg. \ref{alg:eval}, while the results are shown in Table \ref{tab:action_prediction} for both environments.

% \begin{algorithm}[!ht]
% \DontPrintSemicolon
%   \KwInput{EA$^i$, O$^i$, $G_i^t$, $G_i^{t+1}$}
%   \KwOutput{$a^*$}
%   \KwData{Testing set $\mathcal{T}_i \in \mathcal{T}$}
  
%   $z_i = f_\psi ( E_\phi (O^i, EA^i))$\\
%   \text{sample actions $A$ from $\mathcal{U}(0, \text{a}_{max})$} \\
%   \For{a$^j \in A$}    
%         { 
%         	$\hat{G}_i^{j} = g_\theta (G_i^t, a^j, z_i)$ \\
%         	 $e_j = \lVert \hat{G}_i^{j} - G_i^{t+1} \rVert$ \\
%         }
%   $a^* = argmin_{a_j} e_j(G_i^t,G_i^{t+1}, a^j, z_i)$\\
%   $e =  \lVert G_i^{t+1}(a^*) - G_i^{t+1} \rVert$
  

% \caption{Control action prediction}
% \end{algorithm}

% \begin{algorithm}[!ht]
% \DontPrintSemicolon
%   \KwInput{EA$^i$, O$^i$, $G_i^t$, $G_i^{t+1}$}
%   \KwOutput{$a^*$}
%   \KwData{Testing set $\mathcal{T}_i \in \mathcal{T}$}
  
%   $z_i = f_\psi ( E_\phi (O^i, EA^i))$\\
%   \text{sample actions $A$ from $\mathcal{U}(0, \text{a}_{max})$} \\
%   \For{a$^j \in A$}    
%         { 
%         	$\hat{G}_i^{j} = g_\theta (G_i^t, a^j, z_i)$ \\
%         	 $e_j = \lVert \hat{G}_i^{j} - G_i^{t+1} \rVert$ \\
        	 
%               $a^* = argmin_{a_j} e_j(G_i^t,G_i^{t+1}, a^j, z_i)$\\
%               $e_j =  \lVert a^* - a^j \rVert$
%         }
  
% \label{alg:action}
% \caption{Action prediction evaluation}
% \end{algorithm}

% \begin{table}[!h]
%     \centering
%     \caption{Comparison with number of adaptation samples = 3 and dimension of latent space $z_i$ equal to $32$}
%     \begin{tabular}{lcc}\toprule
%          Model & Action Error [N$^2$] & Action Error [mm$^2$] \\
%                 &  Bandaging  &    Lifting           \\
%         \toprule
        
         
%          Baseline               &  14.73   \pm \; \;  22.34     &   1.432 \pm \; \;  2.633  \\ %\toprule
%          Supervised             &  4.06    \pm \; \;  5.617     &   0.0 \pm \; \; 0.0  \\ %\midrule
%          \textbf{Ours}          &  0.066    \pm \; \;  0.291    &   0.065 \pm \; \;  0.284  \\ \bottomrule
%          Oracle                 &  0.267    \pm \; \;  0.533    &   0.0 \pm \; \;  0.0 \\ %\midrule
   
%     \end{tabular}
%     \label{tab:action_prediction}
% \end{table}


\begin{table}[!h]
    \centering
    \caption{Comparison with number of adaptation samples = 5 and dimension of latent space $z_i$ equal to $32$ (NoNorm)}
    \begin{tabular}{lcc}\toprule
         Model & Inverse Model Error  & Inverse Model Error $*10^{-4}$ \\
                &  Bandaging  &    Lifting           \\
        \toprule
        
         
         Baseline               &   \pm \; \;     &   1.1467  \pm \; \;  1.5449  \\ %\toprule
         Supervised             &    \pm \; \;      &  1.0402  \pm \; \; 1.4374 \\ %\midrule
         \textbf{Ours}          &  \pm \; \;      &  0.5012  \pm \; \;   0.2035 \\ \bottomrule
         Oracle                 &     \pm \; \;      &   \pm \; \;  \\ %\midrule
   
    \end{tabular}
    \label{tab:action_prediction}
\end{table}


The results in Table \ref{tab:state_prediction} and Table \ref{tab:action_prediction} show that the proposed model achieves the closest performances to the Oracle model conditioned on the ground-truth parameters. In general, the results show that conditioning on a representation of the physical properties drastically improves the performance in dynamics prediction with respect to an agnostic baseline.
{\comment add about action prediction results ... }

\subsection{Adaptation module evaluation}
% To analyze the representation obtained by the adaptation module, we visualize the projection of the latent space learned for each of the different textile samples $\mathcal{T}_i \in \mathcal{T}$. ({\comment add details of visualization}) Figure \ref{fig:umap} shows the results.
We perform a quantitative evaluation of the quality of the representation extracted by means of a regression task in which the adaptation module trained with our self-supervised method is fine-tuned to predict the ground-truth simulation parameters. The loss used to fine-tune the model is the mean squared error between the prediction of our model and the ground-truth parameters of the simulator {\comment(rewrite better)}. We compare these results with a regressor trained only at predicting the ground-truth parameters. The results are shown in Table \ref{tab:representation_eval}.

\begin{table}[!h]
    \centering
    \caption{Comparison with number of adaptation samples = 1}
    \begin{tabular}{lcc}\toprule
    
         Regressor & Regression Error &  Regression Error  \\
            $z_i$        &  Bandaging  &    Lifting           \\
         
        \toprule
         e2e                            &  1.207    \pm \; \; -    &        0.383  \pm \; \; - \\ \midrule
         supervised                     &  1.026    \pm \; \; -     &         0.411 \pm \; \; - \\ \midrule
         self-supervised (ours)         &   1.205   \pm \; \; -     &        0.441 \pm \; \; - \\ \bottomrule
   
    \end{tabular}
    \label{tab:representation_eval}
\end{table}


\begin{table}[!h]
    \centering
    \caption{Comparison with number of adaptation samples = 1, 3, 5 - NoNorm}
    \begin{tabular}{lcc}\toprule
    
         Regressor & Regression Error &  Regression Error  \\
            $z_i$        &  Bandaging  &    Lifting           \\
         
        \toprule
         e2e                            &  -   \pm \; \; -    &      69.7849    \pm \; \; 95.9333 \\ \midrule
         supervised                     &  -    \pm \; \; -     &         2.7287 \pm \; \; 2.9761 \\ \midrule
         self-supervised (ours)         &  -  \pm \; \; -     &        40.1348 \pm \; \; 37.2678 \\ \midrule
         mean                           & -  \pm \; \; -     &        75.5687 \pm \; \; 62.1949 \\ \bottomrule

        \midrule
         e2e                            & - \pm \; \; -    &        34.7814  \pm \; \; 68.2863 \\ \midrule
         supervised                     &  -    \pm \; \; -     &         0.5604 \pm \; \; 1.033 \\ \midrule
         self-supervised (ours)         &   -   \pm \; \; -     &        31.6727 \pm \; \; 29.7433 \\ \midrule
         mean                           & -  \pm \; \; -     &        75.5687 \pm \; \; 62.1949 \\ \bottomrule

        \bottomrule
         e2e                            & -   \pm \; \; -    &        0.4598  \pm \; \; 0.9782 \\ \midrule
         supervised                     &  - \pm \; \; -     &         0.6001 \pm \; \; 1.009 \\ \midrule
         self-supervised (ours)         &  -  \pm \; \; -     &        23.8968 \pm \; \; 24.5287 \\ \midrule
         mean                           & -  \pm \; \; -     &        75.5687 \pm \; \; 62.1949 \\ \bottomrule
   
    \end{tabular}
    \label{tab:representation_eval}
\end{table}

% \begin{figure}[t!]
%   \centering
%          \includegraphics[width=\linewidth]{images/embedding.png}
%         %  \caption{Prediction of SIM mesh.}
%     \caption{UMAP image}
%     \label{fig:umap}
% \end{figure}

% \begin{figure}[t]
%   \centering
%      \begin{subfigure}[b]{0.45\columnwidth}
%          \centering
%          \includegraphics[width=\linewidth]{images/attention1.png}
%          \caption{Attention on row of nodes in sample 1}
%          \label{fig:rw_profiles}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.49\columnwidth}
%          \centering
%          \includegraphics[width=\linewidth]{images/attention2.png}
%          \caption{Attention in one node in sample 2}
%          \label{fig:rw_profiles}
%      \end{subfigure}
    
%     \vspace{-0.1cm}
%     \caption{Attention examples.}
%     \label{fig:attention}
% \end{figure}

\subsection{Real World evaluation}

To evaluate the capability of the method to work on real data, we replicate the \textit{bandaging task} in the real using two Franka-Emika Panda robots equipped with Optoforce Force/Torque sensors, as visible in Figure~\ref{fig:real_world}. We collect the pulling \ac{ea} and the task trajectories on 40 different textile samples, with the following characteristics (material/construction technique): 8 wool/knitted, 14 cotton/knitted, 4 cotton/woven, 6 polyester/knitted, and 4 polyester/woven (cotton and polyester material classes contain samples with different percentages of elastane). Differently from simulation, the ground-truth physical parameters are not accessible in the real world, as their estimation would require specific tensile tests \cite{} ({\comment from the other paper}). Hence, since the Supervised and Oracle models cannot be trained, we provide the results of the state and action prediction downstream tasks comparing solely against the baseline. The results are visible in Figure \ref{tab:real_world}.

\begin{table}[!h]
    \centering
    \caption{Comparison with number of adaptation samples = 3 and dimension of latent space $z_i$ equal to $8$}
    \begin{tabular}{lcc}\toprule
         Model & State Error [N$^2$] & Action Error [mm$^2$] \\
                &  RW - Bandaging  &    RW - Bandaging        \\
        \toprule
        
         Mean Baseline               &  - \pm \; \;  -    &     - \pm \; \;- \\ %\toprule
         Baseline               &   0.069  \pm \; \;   0.083    &     0.030 \pm \; \; 0.019 \\ %\toprule
         \textbf{Ours}          &   \textbf{0.010}  \pm \; \;   0.008     &   0.024 \pm \; \;  0.014 \\ \bottomrule
   
    \end{tabular}
    \label{tab:real_world}
\end{table}

{\comment Comment on real world results here...}


\subsection{Ablation study}
% {\comment
% Type of experiments that could fit this section:
% \begin{itemize}
%     \item Different "size" of EA (RNN or not as ablation)
%     \item different adjacencies
%     \item no attention VS with attention
%     \item Different types of exploratory action (add bending action results)
%     \item Ground truth graph VS our extraction method
% \end{itemize}

% }

We perform two ablation studies, respectively on the size of the \ac{ea} (Table ~\ref{tab:num_adapt_step}) and on different architecture choices (Table ~\ref{tab:ablation}). 

We do not appreciate particular improvements in performance by increasing the size of \ac{ea}, suggesting that one interaction is enough to obtain the necessary information for the adaptation module {\comment (this might change for the real world case, but in general we have to decide if we want to keep the RNN or not given these results)}. 
% This however might be dependent on the considered case, since the simulator have a lower variance in the behaviours shown with respect to the real case, hence it's easier for the model to learn how to distinguish between different samples. 

In terms of ablation on different architectures, first we evaluate the influence of the attention layer of the adaptation module by substituting it with a simple sum over the features of the embedding for each node. 
{\comment This causes a considerable drop in performance ...

Ablation on multi-hop ... }


\begin{table}[!h]
    \centering
    \caption{Comparison of different adaptation sizes}
    \begin{tabular}{lccc}\toprule
    
         \ac{ea} & State Error [mm$^2$]  &  State Error [mm$^2$]  &  State Error [mm$^2$] \\
            size        &  Bandaging  &    Lifting       &    Real World    \\
         
        \toprule
         1              &  0.133 \pm\;\; 0.168    &   0.085    \pm\;\; 0.058  &   0.016    \pm\;\; 0.023 \\ \midrule
         3              &  0.153 \pm\;\; 0.313    &   0.074    \pm\;\; 0.042  &   0.016    \pm\;\; 0.016\\ \midrule
         5              &  0.116 \pm\;\; 0.138    &   0.086    \pm\;\; 0.061  &   0.010  \pm\;\; 0.008 \\ \bottomrule
   
    \end{tabular}
    \label{tab:num_adapt_step}
\end{table}


% \begin{table}[!h]
%     \centering
%     \caption{Comparison of different adaptation sizes}
%     \begin{tabular}{lccc}\toprule
    
%          \ac{ea} & State Error $*10e^{-3}$  &  State Error $*10^{-3}$  &  State Error $*10^{-3}$ \\
%             size        &  Bandaging  &    Lifting       &    Real World    \\
         
%         \toprule
%          1              &  - \pm\;\; -    &   0.1705    \pm\;\; 0.1060  &   -    \pm\;\; - \\ \midrule
%          3              &  - \pm\;\;  -   &   0.1096    \pm\;\; 0.0414  &   -    \pm\;\; -\\ \midrule
%          5              &  - \pm\;\; -    &   0.1021    \pm\;\; 0.0684  &   -  \pm\;\; - \\ \bottomrule
   
%     \end{tabular}
%     \label{tab:num_adapt_step}
% \end{table}



\begin{table}[!h]
    \centering
    \caption{Ablation study on the components of the model}
    \begin{tabular}{lccc}\toprule
         Model & State Error [mm] &  State Error [mm] &  State Error [mm] \\
                &  Bandaging &    Lifting            &    Real World \\
        \toprule
        
         No attention       & 4.238           \pm\;\; 8.766  & 0.101         \pm\;\; 0.061 & 0.019    \pm\;\; 0.019 \\ %\toprule
         No multi-hop       &  \textbf{0.121} \pm\;\; 0.105  & 0.093         \pm\;\; 0.063 & 0.014  \pm\;\; 0.007 \\ %\midrule
         \textbf{Ours}      &  0.133          \pm\;\; 0.168  & \textbf{0.085}\pm\;\; 0.058 &    0.013  \pm\;\; 0.009 \\ \bottomrule
   
    \end{tabular}
    \label{tab:ablation}
\end{table}



\begin{algorithm}[!ht]

%\begin{multicols}{2}
\DontPrintSemicolon
%   \KwInput{tasks $\mathcal{T}_i \sim \mathcal{T}$, $i \in [1, N_k]$}
%   \KwInput{interactions dataset $\mathcal{D} = \{\mathcal{D}_i\}_ { i \in [1, N_k]} $}
%   \KwOutput{$a^*$}
  \KwData{Testing tasks $\mathcal{T}_i \sim \mathcal{T}$, $i \in [1, N_k]$}
  \KwData{Interactions dataset $\mathcal{D} = \{\mathcal{D}_i\}_ { i \in [1, N_k]} $}
  \KwData{Actions distribution $\mathcal{A}$}
  \KwData{Goals distribution $Goals = \{a_j, goal_j\}_ { i \in [1, N_j]} $}
  \;
  
  % Set Function Names
  \SetKwFunction{FEvaluate}{Main}
  \SetKwFunction{FAdapt}{adapt}
  \SetKwFunction{FForward}{forward}
  \SetKwFunction{FAction}{getAction}

   % Write Function with word ``Function''

  \For{ $\mathcal{T}_i \sim \mathcal{T}$}    
        {   \rule{0pt}{1ex} \; 
            \underline{\textbf{adapt}} \;
            $\mathcal{D}^{EA^i}=\{G_t^i, F_t^i\}_{t = 1,...,T}$        \tcp*{execute $EA^i$}
            $\mathcal{D}^{A^i}=\{G_a^i, F_a^i\}_{a= 1,...,n_a} \sim \mathcal{D}^{EA^i} $\;
            $z_i = f_\phi(\{\mathcal{D}^{A^i}, z_0)$\;
            % FORWARD EVAL
            \rule{0pt}{1ex}  \; 
            \underline{\textbf{forward dynamics (state prediction)}} \;
            $e_g^i = 0$            \tcp*{graph  error}                                             
             \For{$\{G_t^i, a^t\}\sim \mathcal{D}_i$}    
                { 
                     $\hat{G}_i^{t+1} = g_\theta (G_i^t, a^t, z_i)$ \;
                	 $e_g^i +=  \lVert \hat{G}_i^{t+1} - G_i^{t+1} \rVert$\;
                }
                \rule{0pt}{1ex}  \; 
            % ACTION EVAL
            \underline{\textbf{action prediction}}\; 
            $e_a^i = 0$            \tcp*{action  error}                                             
             \For{$a^j, Goal_j \sim Goals$}    
                {   
                    $G_t^i \sim \mathcal{D}_i$\;
                	\For{a$^j \sim A$}    
                    { 
                    	$\hat{G}_i^{j} = g_\theta (G_i^t, a^j, z_i)$ \;
                    	 $\hat{G}oal_i^{j} \xleftarrow[]{} \hat{G}_i^{j}$\;
                    	 $e_j = \lVert \hat{G}oal_i^{j} - Goal_i^{j} \rVert$ \;
                    }
  
                    $a^* = argmin_{a_j} e_j$ \;
                	 $e_a^i += \lVert a^* - a^j \rVert$\;
                }
            
        }
  

  \;
  
    
\caption{Adaptation evaluation}

%\end{multicols}
\label{alg:eval}
\end{algorithm}






% \begin{algorithm}[!ht]

% %\begin{multicols}{2}
% \DontPrintSemicolon
% %   \KwInput{tasks $\mathcal{T}_i \sim \mathcal{T}$, $i \in [1, N_k]$}
% %   \KwInput{interactions dataset $\mathcal{D} = \{\mathcal{D}_i\}_ { i \in [1, N_k]} $}
% %   \KwOutput{$a^*$}
%   \KwData{Testing tasks $\mathcal{T}_i \sim \mathcal{T}$, $i \in [1, N_k]$}
%   \KwData{Interactions dataset $\mathcal{D} = \{\mathcal{D}_i\}_ { i \in [1, N_k]} $}
%   \KwData{Actions distribution $\mathcal{A}$}
%   \KwData{Goals distribution $Goals = \{a_j, goal_j\}_ { i \in [1, N_j]} $}
%   \;
  
%   % Set Function Names
%   \SetKwFunction{FEvaluate}{Main}
%   \SetKwFunction{FAdapt}{adapt}
%   \SetKwFunction{FForward}{forward}
%   \SetKwFunction{FAction}{getAction}
  
%   % Write Function with word ``Function''
%   \SetKwProg{Fn}{Def}{:}{}
%   \Fn{\FAdapt{$\mathcal{T}_i$, $z_0$}}{
%     $\mathcal{D}^{EA^i}=\{G_t^i, F_t^i\}_{t = 1,...,T}$        \tcp*{execute $EA^i$}
%     $\mathcal{D}^{A^i}=\{G_a^i, F_a^i\}_{a= 1,...,n_a} \sim \mathcal{D}^{EA^i} $\;
%     $z_i = f_\phi(\{\mathcal{D}^{A^i}, z_0)$\;
%     \KwRet $z_i$
%   }\;
  
%   % Write Function with word ``Function''
%   \SetKwProg{Fn}{Def}{:}{}
%   \Fn{\FForward{$G_t^i, a^t, z_i$}}{
%     $\hat{G}_i^{t+1} = g_\theta (G_i^t, a^t, z_i)$ \;
%     \KwRet $\hat{G}_i^{t+1}$\;
%   }
%   \;
  
%     % Write Function with word ``Function''
%   \SetKwProg{Fn}{Def}{:}{}
%   \Fn{\FAction{$Goal^i, G_t^i, z_i$}}{
%   \For{a$^j \sim A$}    
%         { 
%         	$\hat{G}_i^{j} = g_\theta (G_i^t, a^j, z_i)$ \;
%         	 $\hat{G}oal_i^{j} \xleftarrow[]{} \hat{G}_i^{j}$\;
%         	 $e_j = \lVert \hat{G}oal_i^{j} - Goal_i^{j} \rVert$ \;
%         }
  
%     $a^* = argmin_{a_j} e_j$ \;
%     \KwRet $a^* $\;
%   }
%   \;
%   \pagebreak
%   % Write Function with word ``Function''
%   \SetKwProg{Fn}{Function}{:}{}
%   \Fn{\FEvaluate}{
%   \For{ $\mathcal{T}_i \sim \mathcal{T}$}    
%         { 
%             $z_i = $ adapt($\mathcal{T}_i$, $z_0$)\;
%             % FORWARD EVAL
%             $e_g^i = 0$            \tcp*{graph prediciton error}                                             
%              \For{$\{G_t^i, a^t\}\sim \mathcal{D}_i$}    
%                 { 
%                 	$\hat{G}_i^{j} = $ forward$(G_t^i, a^t, z_i)$\;
%                 	 $e_g^i +=  \lVert \hat{G}_i^{t+1} - G_i^{t+1} \rVert$\;
%                 }
%             % ACTION EVAL
%             $e_a^i = 0$            \tcp*{action prediciton error}                                             
%              \For{$a^j, Goal_j \sim Goals$}    
%                 {   
%                     $G_t^i \sim \mathcal{D}_i$\;
%                 	$a^* =$ getAction$(Goal_j, G_t^i, z_i)$\;
%                 	 $e_a^i += \lVert a^* - a^j \rVert$\;
%                 }
            
%         }
  
  
%   }
%   \;
  

% \label{alg:action}
% \caption{Adaptation evaluation}

% %\end{multicols}
% \end{algorithm}


==> sections/old/05_experiments_inverse.tex <==


\section{Experiments}
In this section we want to evaluate the capability of the learned latent representation $z_i$ and of the forward model $g_\theta$ to generalize over a variety of physical properties of cloth-like deformable objects, in both simulation environments as well as in the real world.
%The experimental evaluation aims at showing the capability of the proposed model to learn how to generalize over a variety of physical properties of deformable objects influencing their dynamics. We evaluate both the performance of the forward dynamics model and the quality of the adaptation module in learning a representation $z_i$ of the physical properties. 
To this aim, we carry the following evaluations:
\begin{enumerate}
    \item We test the performance of the forward dynamics module in a state prediction downstream task over a set of deformable objects $\mathcal{T}_i \sim \mathcal{T}$ with \emph{unseen} elastic physical properties $i$. 
    % \item We qualitatively evaluate the learned representation by visualizing a UMAP projection of the latent space of the learned parameters.
    \item We quantitatively evaluate whether the learned representation encodes information about deformable object physical properties by learning an inverse model conditioned on the learned representation $z_i$ to predict the control action between two states.
    \item We  examine in simulation how accurately we can decode physical properties from the learned representation by learning a regressor of the ground-truth parameters on top of the learned representation $z_i$.
    \item We carry an ablation study on the influence of the length $T$ of the sequence of observations $O^i$ to encode $z_i$ {\comment, and on the architectural choices for the overall model}. 
    % {(\comment also type of \ac{ea} if we have the time)}.
\end{enumerate}



\subsection{Forward module evaluation}
% \subsection{Algorithm experiments}
The forward dynamics module receives the initial observation of the cloth $G_i^t$ and the control action $a_t$, and is asked to predict the graph at the following time step $G_i^{t+1}$. The performance is the mean square error computed between the graph $G_i^{t+1}$ and the graph predicted by the model $\hat{G}_i^{t+1}$. The control action $a_t$ is different for the two environments: in \textit{partial bandage}, $a_t$ is the force perceived by the end-effectors when $G_i^{t+1}$ is reached, while in \textit{lifting} $a_t$ is the altitude at which the end-effectors are moved. The pseudo code of the algorithm can be seen in Alg. \ref{alg:eval}, while the results are shown in Table \ref{tab:state_prediction} for both environments. 
We compare the performance of the forward dynamics module with the following models:
\begin{enumerate}
    \item \textbf{Not conditioned (NC):} $g_\theta$ is trained to predict $\hat{G}_i^{t+1}$ given only the initial state $G_t$ and the action $a_t$, without any conditioning on $z_i$. 
    \item \textbf{Supervised (Sup):} $g_\theta$ is trained to predict $\hat{G}_i^{t+1}$ while $f_\phi$ is also trained to predict the ground-truth simulation parameters \textit{i}. 
    \item \textbf{Self-supervised - T=1 (SS1):} 
    \item \textbf{Self-supervised - T=10 (ElasNet):} 
    \item \textbf{Oracle:} the forward model $g_\theta$ is conditioned on the ground-truth simulation parameters.
\end{enumerate}

% \begin{algorithm}[!ht]
% \DontPrintSemicolon
%   \KwInput{EA$^i$, O$^i$, $a^t$, $G_i^t$}
%   \KwOutput{$\hat{G}_i^{t+1}$}
%   \KwData{Testing set $\mathcal{T}_i \in \mathcal{T}$}
  
%   $z_i = f_\psi ( E_\phi (O^i, EA^i))$\\
%   $\hat{G}_i^{t+1} = g_\theta (G_i^t, a^t, z_i)$ \\
%   $e = \lVert \hat{G}_i^{t+1} - G_i^{t+1} \rVert$ \\
 
% \label{alg:state}
% \caption{State prediction evaluation}
% \end{algorithm}

% \begin{table}[!h]
%     \centering
%     \caption{Comparison with number of adaptation samples =3 }
%     \begin{tabular}{lcc}\toprule
%          Model & State Error [mm$^2$] &  State Error [mm$^2$]   \\
%                 &  Bandaging  &    Lifting                      \\
%         \toprule
        
%          Baseline               &  4.229            \pm \; \;   8.923   & 3.323             \pm \; \;   6.566     \\ %\toprule
%          Supervised             &  0.928            \pm \; \;   1.579   & 0.099             \pm \; \;  0.045        \\ %\midrule
%          \textbf{Ours}          &  \textbf{0.133}   \pm \; \;   0.168   & \textbf{0.085}    \pm \; \; \textbf{0.058}\\ \bottomrule
%          Oracle                 &  0.103            \pm \; \;   0.099   & 0.074           \pm \; \;    0.040        \\ %\midrule
   
%     \end{tabular}
%     \label{tab:state_prediction}
% \end{table}

\begin{table}[!h]
    \centering
    \caption{Comparison with number of adaptation samples = 5 }
    \begin{tabular}{lcc}\toprule
         Model & State Error $*10^{-3}$ &  State Error $*10^{-3}$    \\
                &  Partial bandage  &    Lifting                      \\
        \toprule
        
         NC               &  29.6032            \pm \; \;   65.2891   &    6.5845         \pm \; \;    12.786    \\ %\toprule
         Sup             &  0.9921            \pm \; \;   1.47972   &    0.3211           \pm \; \;  0.6993        \\ %\midrule
         SS1             &  0.2599            \pm \; \;   0.1965   &    0.1705           \pm \; \;  0.1060        \\ %\midrule
         \textbf{ElasNet}          &  \textbf{0.1505}             \pm \; \;   \textbf{0.1247}   &   \textbf{0.1020}    \pm\;\; \textbf{0.0684} \\ \bottomrule
         Oracle                 &  0.1216            \pm \; \;   0.1943   &     0.0808      \pm \; \;     0.0399       \\ %\midrule
   
    \end{tabular}
    \label{tab:state_prediction}
\end{table}


\subsection{Adaptation model evaluation}

\begin{figure}[t!]
  \centering
         \includegraphics[width=\linewidth]{images/evaluation.pdf}
        %  \caption{Prediction of SIM mesh.}
    \caption{Evaluation experiments of the quality of the learned adaptive representation $z_i$. {\comment probably to be remvoved}}
    \label{fig:eval}
\end{figure}

In this section we aim to evaluate the quality of the learned representation $z_i$ extracted from the adaptation module $f_\phi$ by answering the following questions: 1) is it possible to decode from the latent representation $z_i$ the ground truth physical parameters of the deformable object $\mathcal{T}_i$? 2) does the latent representation generalize to a different downstream tasks such as learning inverse dynamics of different elastic samples? 3) does the latent representation transfer its performance across different environments?
To address these questions we focus on the representation learned form the \emph{partial bandage} environment and we design three experiments, visualized in Fig.~\ref{fig:eval}. The first experiment (\emph{regressor}) evaluate how accurately it is possible to decode the ground truth physical properties of different $\mathcal{T}_i$ from $z_i$. In particular, we train a network  $r_\gamma$ implemented as an \ac{mlp} with 3 hidden layers of size 64 and ReLU non-linearities to regress the bending $b_i$ and elastic $k_i$ parameters of the simulator for the testing samples. We compare the predictions obtained form the learned representation of our model with a model learned form the latent representation of the \textbf{SS} model, a model that learns end-to-end the predictions (\textbf{e2e}) and the mean prediction. 

\begin{table}[!h]
    \centering
    \caption{Physical parameters ($k_i, b_i$) prediction for test $\mathcal{T}_i$ not seen during training.}
    \begin{tabular}{lcc}\toprule
         Model & MSE - $k_i$ &  MSE - $b_i$    \\
        \toprule
        
         mean               &  0.718            \pm \; \;   0.604   &    0.501       \pm \; \;   0.500    \\ %\toprule
         e2e             &  0.180            \pm \; \;   0.305   &    0.128           \pm \; \;  0.201        \\ %\midrule
         Sup             &  0.231            \pm \; \;   0.209   &    0.291           \pm \; \;  0.291        \\ %\midrule
         \textbf{ElasNet}          &  0.276             \pm \; \;   0.254   &  0.329   \pm\;\; 0.314 \\ \bottomrule
   
    \end{tabular}
    \label{tab:regressor}
\end{table}

Table~\ref{tab:regressor} shows that .... {\comment fill in results}
The second (\emph{Inverse Dynamics}) and third (\emph{Lifting Environment}) experiments aim at showing the quality of the learned representation by using it for different downstream tasks which are respectively an inverse dynamics task for the same environment (arm) or a forward dynamics task in a different environment (lifting). 
In particular, the \emph{Inverse Dynamics} experiment trains an inverse dynamics model $i_\beta$ conditioned on the adapted $z_i$ to predict the control action $a_i^{t}$ between the initial state of the deformable object $G_0^i$ and a second state $G_t^i$. We architecture of the dynamics model is composed by a node and pysical properties encoder implemented as \ac{mlp}s, where we obtain the final action prediction by applying a linear projection to the concatenation of the action and the nodes and aggregating the nodes with the average aggregation.  The performance of the model is evaluated by computing the mean squared error between the predicted action $\hat{a}_i^{t}$ and the ground-truth action $a_i^{t}$. We compare the inverse model learned on the latent representation extracted from our method (\textbf{ElasNet}) with the one learned from the \textbf{Sup} model, one conditioned on the ground truth parameters (\textbf{Oracle}) and a non-conditioned (\textbf{NC}) inverse model.  For what concern the \emph{Lifting Environment} experiment, we take the forward dynamics model $g_{\theta}$ and the adatation model $f_\phi$ trained on the \emph{partial bendage} environment and we fine-tune forward dynamics model while keeping fixed the weights of $f_\phi$ to learn the \emph{lifting} environment. We compare the performance of the model fine-tuned from \textbf{ElasNet} with the one fine-tuned from the \textbf{Sup} and the oracle and baseline performance which in our case are the \textbf{NC} and \textbf{ElasNet} models trained directly on the \emph{lifting} environment.


\begin{table}[!h]
    \centering
    \caption{Comparison with $T=5$ and dimension of latent space $z_i$ equal to $32$. {\comment make this figure as an histogram}}
    \begin{tabular}{lcc}\toprule
         Model & Inverse Model Error & Forward Model Error $*10^{-3}$ \\
                &  Bandaging  &    Lifting           \\
        \toprule
        
         
         NC               &  9.2717 \pm \; \;  10.6463   &    6.5845         \pm \; \;    12.786  \\ %\toprule
         Sup             &   0.0502 \pm \; \;  0.0545    &   0.350 \pm \; \; 0.601 \\ %\midrule
         \textbf{ElasNet}          &   0.0376 \pm \; \;   0.0303   &  0.152  \pm \; \;   0.146 \\ \bottomrule
         Oracle                 &  0.0789   \pm \; \;   0.0664   &   0.1020    \pm\;\; 0.0684 \\ %\midrule
   
    \end{tabular}
    \label{tab:inverse_model}
\end{table}

Table~\ref{tab:inverse_model} shows ....



% \subsection{Inverse model evaluation}




% In the inverse model evaluation, instead, an inverse dynamics model receives both the initial observation of the cloth $G_0$ and a second state $G_t$, and is trained to predict the control action $a_i^{t}$ between them. The performance is the mean square error computed between the predicted action $\hat{a}_i^{t}$ and the ground-truth action $a_i^{t}$ {(\comment details of the model in the appendix?)}. The pseudo code of the algorithm can be seen in Alg. \ref{alg:eval}, while the results are shown in Table \ref{tab:state_prediction} for both environments. 

% \begin{algorithm}[!ht]
% \DontPrintSemicolon
%   \KwInput{EA$^i$, O$^i$, $G_i^t$, $G_i^{t+1}$}
%   \KwOutput{$a^*$}
%   \KwData{Testing set $\mathcal{T}_i \in \mathcal{T}$}
  
%   $z_i = f_\psi ( E_\phi (O^i, EA^i))$\\
%   \text{sample actions $A$ from $\mathcal{U}(0, \text{a}_{max})$} \\
%   \For{a$^j \in A$}    
%         { 
%         	$\hat{G}_i^{j} = g_\theta (G_i^t, a^j, z_i)$ \\
%         	 $e_j = \lVert \hat{G}_i^{j} - G_i^{t+1} \rVert$ \\
%         }
%   $a^* = argmin_{a_j} e_j(G_i^t,G_i^{t+1}, a^j, z_i)$\\
%   $e =  \lVert G_i^{t+1}(a^*) - G_i^{t+1} \rVert$
  

% \caption{Control action prediction}
% \end{algorithm}

% \begin{algorithm}[!ht]
% \DontPrintSemicolon
%   \KwInput{EA$^i$, O$^i$, $G_i^t$, $G_i^{t+1}$}
%   \KwOutput{$a^*$}
%   \KwData{Testing set $\mathcal{T}_i \in \mathcal{T}$}
  
%   $z_i = f_\psi ( E_\phi (O^i, EA^i))$\\
%   \text{sample actions $A$ from $\mathcal{U}(0, \text{a}_{max})$} \\
%   \For{a$^j \in A$}    
%         { 
%         	$\hat{G}_i^{j} = g_\theta (G_i^t, a^j, z_i)$ \\
%         	 $e_j = \lVert \hat{G}_i^{j} - G_i^{t+1} \rVert$ \\
        	 
%               $a^* = argmin_{a_j} e_j(G_i^t,G_i^{t+1}, a^j, z_i)$\\
%               $e_j =  \lVert a^* - a^j \rVert$
%         }
  
% \label{alg:action}
% \caption{Action prediction evaluation}
% \end{algorithm}

% \begin{table}[!h]
%     \centering
%     \caption{Comparison with number of adaptation samples = 3 and dimension of latent space $z_i$ equal to $32$}
%     \begin{tabular}{lcc}\toprule
%          Model & Action Error [N$^2$] & Action Error [mm$^2$] \\
%                 &  Bandaging  &    Lifting           \\
%         \toprule
        
         
%          Baseline               &  14.73   \pm \; \;  22.34     &   1.432 \pm \; \;  2.633  \\ %\toprule
%          Supervised             &  4.06    \pm \; \;  5.617     &   0.0 \pm \; \; 0.0  \\ %\midrule
%          \textbf{Ours}          &  0.066    \pm \; \;  0.291    &   0.065 \pm \; \;  0.284  \\ \bottomrule
%          Oracle                 &  0.267    \pm \; \;  0.533    &   0.0 \pm \; \;  0.0 \\ %\midrule
   
%     \end{tabular}
%     \label{tab:action_prediction}
% \end{table}




% {\comment (comment on results of fwd and inv models) The results in Table \ref{tab:state_prediction} and Table \ref{tab:action_prediction} show that the proposed model achieves the closest performances to the Oracle model conditioned on the ground-truth parameters. In general, the results show that conditioning on a representation of the physical properties drastically improves the performance in dynamics prediction with respect to an agnostic baseline. }

% \subsection{Adaptation module evaluation}
% To analyze the representation obtained by the adaptation module, we visualize the projection of the latent space learned for each of the different textile samples $\mathcal{T}_i \in \mathcal{T}$. ({\comment add details of visualization}) Figure \ref{fig:umap} shows the results.
% We perform a quantitative evaluation of the quality of the representation extracted by means of a regression task in which the adaptation module trained with our self-supervised method is fine-tuned to predict the ground-truth simulation parameters. The loss used to fine-tune the model is the mean squared error between the prediction of our model and the ground-truth parameters of the simulator {\comment(rewrite better)}. We compare these results with a regressor trained only at predicting the ground-truth parameters. The results are shown in Table \ref{tab:representation_eval}.

% \begin{table}[!h]
%     \centering
%     \caption{Comparison with number of adaptation samples = 1}
%     \begin{tabular}{lcc}\toprule
    
%          Regressor & Regression Error &  Regression Error  \\
%             $z_i$        &  Bandaging  &    Lifting           \\
         
%         \toprule
%          e2e                            &  1.207    \pm \; \; -    &        0.383  \pm \; \; - \\ \midrule
%          supervised                     &  1.026    \pm \; \; -     &         0.411 \pm \; \; - \\ \midrule
%          self-supervised (ours)         &   1.205   \pm \; \; -     &        0.441 \pm \; \; - \\ \bottomrule
   
%     \end{tabular}
%     \label{tab:representation_eval}
% \end{table}
\subsection{Support size evaluation}
In this section we carry an ablation study on the role of the length of the sequence of observations $T$ to adapt the latente representation $z_i$. 
\begin{table}[!h]
    \centering
    \caption{Comparison with number of adaptation samples = 1, 3, 5 - NoNorm}
    \begin{tabular}{lcc}\toprule
    
         Regressor & Regression Error &  Regression Error  \\
            $z_i$        &  Bandaging  &    Lifting           \\
         
        \toprule
         e2e                            &  38.002   \pm \; \; 63.1359    &      69.7849    \pm \; \; 95.9333 \\ \midrule
         supervised                     &  44.1783    \pm \; \; 61.3092     &         2.7287 \pm \; \; 2.9761 \\ \midrule
         self-supervised (ours)         &  38.6822  \pm \; \; 35.6275     &        40.1348 \pm \; \; 37.2678 \\ \midrule
         mean                           & 75.5687  \pm \; \; 62.1949      &        75.5687 \pm \; \; 62.1949 \\ \bottomrule

        \midrule
         e2e                            & 31.5563 \pm \; \; 59.9998    &        34.7814  \pm \; \; 68.2863 \\ \midrule
         supervised                     &  41.7757    \pm \; \; 68.0116     &         0.5604 \pm \; \; 1.033 \\ \midrule
         self-supervised (ours)         &   35.0488   \pm \; \; 30.3957     &        31.6727 \pm \; \; 29.7433 \\ \midrule
         mean                           & 75.5687  \pm \; \; 62.1949   &        75.5687 \pm \; \; 62.1949 \\ \bottomrule

        \bottomrule
         e2e                            & 18.5594   \pm \; \; 28.1066    &        0.4598  \pm \; \; 0.9782 \\ \midrule
         supervised                     &  23.3779 \pm \; \; 43.4261     &         0.6001 \pm \; \; 1.009 \\ \midrule
         self-supervised (ours)         &  21.9112  \pm \; \; 26.8477     &        23.8968 \pm \; \; 24.5287 \\ \midrule
         mean                           & 75.5687 \pm \; \; 62.1949    &        75.5687 \pm \; \; 62.1949 \\ \bottomrule
   
    \end{tabular}
    \label{tab:representation_eval}
\end{table}

% \begin{figure}[t!]
%   \centering
%          \includegraphics[width=\linewidth]{images/embedding.png}
%         %  \caption{Prediction of SIM mesh.}
%     \caption{UMAP image}
%     \label{fig:umap}
% \end{figure}

% \begin{figure}[t]
%   \centering
%      \begin{subfigure}[b]{0.45\columnwidth}
%          \centering
%          \includegraphics[width=\linewidth]{images/attention1.png}
%          \caption{Attention on row of nodes in sample 1}
%          \label{fig:rw_profiles}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.49\columnwidth}
%          \centering
%          \includegraphics[width=\linewidth]{images/attention2.png}
%          \caption{Attention in one node in sample 2}
%          \label{fig:rw_profiles}
%      \end{subfigure}
    
%     \vspace{-0.1cm}
%     \caption{Attention examples.}
%     \label{fig:attention}
% \end{figure}

\subsection{Real World evaluation}

To evaluate the capability of the method to work on real data,
...
Differently from simulation, the ground-truth physical parameters are not accessible in the real world, as their estimation would require specific tensile tests \cite{} ({\comment from the other paper}). Hence, since the Supervised and Oracle models cannot be trained, we provide the results of the state and action prediction downstream tasks comparing solely against the baseline. The results are visible in Figure \ref{tab:real_world}.

\begin{table}[!h]
    \centering
    \caption{Comparison with number of adaptation samples = 3 and dimension of latent space $z_i$ equal to $8$}
    \begin{tabular}{lcc}\toprule
         Model & Forward Dynamics MSE & Inverse Dynamics MSE \\
                &  RW - Bandaging  &    RW - Bandaging        \\
        \toprule
        
         Mean Baseline               &  - \pm \; \;  -    &     - \pm \; \;- \\ %\toprule
         Baseline               &   0.069  \pm \; \;   0.083    &     0.030 \pm \; \; 0.019 \\ %\toprule
         \textbf{Ours}          &   \textbf{0.010}  \pm \; \;   0.008     &   0.024 \pm \; \;  0.014 \\ \bottomrule
   
    \end{tabular}
    \label{tab:real_world}
\end{table}

{\comment Comment on real world results here...}


\subsection{Ablation study}
% {\comment
% Type of experiments that could fit this section:
% \begin{itemize}
%     \item Different "size" of EA (RNN or not as ablation)
%     \item different adjacencies
%     \item no attention VS with attention
%     \item Different types of exploratory action (add bending action results)
%     \item Ground truth graph VS our extraction method
% \end{itemize}

% }

We perform two ablation studies, respectively on the size of the \ac{ea} (Table ~\ref{tab:num_adapt_step}) and on different architecture choices (Table ~\ref{tab:ablation}). 

We do not appreciate particular improvements in performance by increasing the size of \ac{ea}, suggesting that one interaction is enough to obtain the necessary information for the adaptation module {\comment (this might change for the real world case, but in general we have to decide if we want to keep the RNN or not given these results)}. 
% This however might be dependent on the considered case, since the simulator have a lower variance in the behaviours shown with respect to the real case, hence it's easier for the model to learn how to distinguish between different samples. 

In terms of ablation on different architectures, first we evaluate the influence of the attention layer of the adaptation module by substituting it with a simple sum over the features of the embedding for each node. 
{\comment This causes a considerable drop in performance ...

Ablation on multi-hop ... }


\begin{table}[!h]
    \centering
    \caption{Comparison of different adaptation sizes}
    \begin{tabular}{lccc}\toprule
    
         \ac{ea} & State Error [mm$^2$]  &  State Error [mm$^2$]  &  State Error [mm$^2$] \\
            size        &  Bandaging  &    Lifting       &    Real World    \\
         
        \toprule
         1              &  0.133 \pm\;\; 0.168    &   0.085    \pm\;\; 0.058  &   0.016    \pm\;\; 0.023 \\ \midrule
         3              &  0.153 \pm\;\; 0.313    &   0.074    \pm\;\; 0.042  &   0.016    \pm\;\; 0.016\\ \midrule
         5              &  0.116 \pm\;\; 0.138    &   0.086    \pm\;\; 0.061  &   0.010  \pm\;\; 0.008 \\ \bottomrule
   
    \end{tabular}
    \label{tab:num_adapt_step}
\end{table}


% \begin{table}[!h]
%     \centering
%     \caption{Comparison of different adaptation sizes}
%     \begin{tabular}{lccc}\toprule
    
%          \ac{ea} & State Error $*10e^{-3}$  &  State Error $*10^{-3}$  &  State Error $*10^{-3}$ \\
%             size        &  Bandaging  &    Lifting       &    Real World    \\
         
%         \toprule
%          1              &  - \pm\;\; -    &   0.1705    \pm\;\; 0.1060  &   -    \pm\;\; - \\ \midrule
%          3              &  - \pm\;\;  -   &   0.1096    \pm\;\; 0.0414  &   -    \pm\;\; -\\ \midrule
%          5              &  - \pm\;\; -    &   0.1021    \pm\;\; 0.0684  &   -  \pm\;\; - \\ \bottomrule
   
%     \end{tabular}
%     \label{tab:num_adapt_step}
% \end{table}



\begin{table}[!h]
    \centering
    \caption{Ablation study on the components of the model}
    \begin{tabular}{lccc}\toprule
         Model & State Error [mm] &  State Error [mm] &  State Error [mm] \\
                &  Bandaging &    Lifting            &    Real World \\
        \toprule
        
         No attention       & 4.238           \pm\;\; 8.766  & 0.101         \pm\;\; 0.061 & 0.019    \pm\;\; 0.019 \\ %\toprule
         No multi-hop       &  \textbf{0.121} \pm\;\; 0.105  & 0.093         \pm\;\; 0.063 & 0.014  \pm\;\; 0.007 \\ %\midrule
         \textbf{Ours}      &  0.133          \pm\;\; 0.168  & \textbf{0.085}\pm\;\; 0.058 &    0.013  \pm\;\; 0.009 \\ \bottomrule
   
    \end{tabular}
    \label{tab:ablation}
\end{table}



\begin{algorithm}[!ht]

%\begin{multicols}{2}
\DontPrintSemicolon
%   \KwInput{tasks $\mathcal{T}_i \sim \mathcal{T}$, $i \in [1, N_k]$}
%   \KwInput{interactions dataset $\mathcal{D} = \{\mathcal{D}_i\}_ { i \in [1, N_k]} $}
%   \KwOutput{$a^*$}
  \KwData{Testing tasks $\mathcal{T}_i \sim \mathcal{T}$, $i \in [1, N_k]$}
  \KwData{Interactions dataset $\mathcal{D} = \{\mathcal{D}_i\}_ { i \in [1, N_k]} $}
  \KwData{Actions distribution $\mathcal{A}$}
  \KwData{Goals distribution $Goals = \{a_j, goal_j\}_ { i \in [1, N_j]} $}
  \;
  
  % Set Function Names
  \SetKwFunction{FEvaluate}{Main}
  \SetKwFunction{FAdapt}{adapt}
  \SetKwFunction{FForward}{forward}
  \SetKwFunction{FAction}{getAction}

   % Write Function with word ``Function''

  \For{ $\mathcal{T}_i \sim \mathcal{T}$}    
        {   \rule{0pt}{1ex} \; 
            \underline{\textbf{adapt}} \;
            $\mathcal{D}^{EA^i}=\{G_t^i, F_t^i\}_{t = 1,...,T}$        \tcp*{execute $EA^i$}
            $\mathcal{D}^{A^i}=\{G_a^i, F_a^i\}_{a= 1,...,n_a} \sim \mathcal{D}^{EA^i} $\;
            $z_i = f_\phi(\{\mathcal{D}^{A^i}, z_0)$\;
            % FORWARD EVAL
            \rule{0pt}{1ex}  \; 
            \underline{\textbf{forward dynamics (state prediction)}} \;
            $e_g^i = 0$            \tcp*{graph  error}                                             
             \For{$\{G_t^i, a^t\}\sim \mathcal{D}_i$}    
                { 
                     $\hat{G}_i^{t+1} = g_\theta (G_i^t, a^t, z_i)$ \;
                	 $e_g^i +=  \lVert \hat{G}_i^{t+1} - G_i^{t+1} \rVert$\;
                }
                \rule{0pt}{1ex}  \; 
            % ACTION EVAL
            \underline{\textbf{action prediction}}\; 
            $e_a^i = 0$            \tcp*{action  error}                                             
             \For{$a^j, Goal_j \sim Goals$}    
                {   
                    $G_t^i \sim \mathcal{D}_i$\;
                	\For{a$^j \sim A$}    
                    { 
                    	$\hat{G}_i^{j} = g_\theta (G_i^t, a^j, z_i)$ \;
                    	 $\hat{G}oal_i^{j} \xleftarrow[]{} \hat{G}_i^{j}$\;
                    	 $e_j = \lVert \hat{G}oal_i^{j} - Goal_i^{j} \rVert$ \;
                    }
  
                    $a^* = argmin_{a_j} e_j$ \;
                	 $e_a^i += \lVert a^* - a^j \rVert$\;
                }
            
        }
  

  \;
  
    
\caption{Adaptation evaluation}

%\end{multicols}
\label{alg:eval}
\end{algorithm}






% \begin{algorithm}[!ht]

% %\begin{multicols}{2}
% \DontPrintSemicolon
% %   \KwInput{tasks $\mathcal{T}_i \sim \mathcal{T}$, $i \in [1, N_k]$}
% %   \KwInput{interactions dataset $\mathcal{D} = \{\mathcal{D}_i\}_ { i \in [1, N_k]} $}
% %   \KwOutput{$a^*$}
%   \KwData{Testing tasks $\mathcal{T}_i \sim \mathcal{T}$, $i \in [1, N_k]$}
%   \KwData{Interactions dataset $\mathcal{D} = \{\mathcal{D}_i\}_ { i \in [1, N_k]} $}
%   \KwData{Actions distribution $\mathcal{A}$}
%   \KwData{Goals distribution $Goals = \{a_j, goal_j\}_ { i \in [1, N_j]} $}
%   \;
  
%   % Set Function Names
%   \SetKwFunction{FEvaluate}{Main}
%   \SetKwFunction{FAdapt}{adapt}
%   \SetKwFunction{FForward}{forward}
%   \SetKwFunction{FAction}{getAction}
  
%   % Write Function with word ``Function''
%   \SetKwProg{Fn}{Def}{:}{}
%   \Fn{\FAdapt{$\mathcal{T}_i$, $z_0$}}{
%     $\mathcal{D}^{EA^i}=\{G_t^i, F_t^i\}_{t = 1,...,T}$        \tcp*{execute $EA^i$}
%     $\mathcal{D}^{A^i}=\{G_a^i, F_a^i\}_{a= 1,...,n_a} \sim \mathcal{D}^{EA^i} $\;
%     $z_i = f_\phi(\{\mathcal{D}^{A^i}, z_0)$\;
%     \KwRet $z_i$
%   }\;
  
%   % Write Function with word ``Function''
%   \SetKwProg{Fn}{Def}{:}{}
%   \Fn{\FForward{$G_t^i, a^t, z_i$}}{
%     $\hat{G}_i^{t+1} = g_\theta (G_i^t, a^t, z_i)$ \;
%     \KwRet $\hat{G}_i^{t+1}$\;
%   }
%   \;
  
%     % Write Function with word ``Function''
%   \SetKwProg{Fn}{Def}{:}{}
%   \Fn{\FAction{$Goal^i, G_t^i, z_i$}}{
%   \For{a$^j \sim A$}    
%         { 
%         	$\hat{G}_i^{j} = g_\theta (G_i^t, a^j, z_i)$ \;
%         	 $\hat{G}oal_i^{j} \xleftarrow[]{} \hat{G}_i^{j}$\;
%         	 $e_j = \lVert \hat{G}oal_i^{j} - Goal_i^{j} \rVert$ \;
%         }
  
%     $a^* = argmin_{a_j} e_j$ \;
%     \KwRet $a^* $\;
%   }
%   \;
%   \pagebreak
%   % Write Function with word ``Function''
%   \SetKwProg{Fn}{Function}{:}{}
%   \Fn{\FEvaluate}{
%   \For{ $\mathcal{T}_i \sim \mathcal{T}$}    
%         { 
%             $z_i = $ adapt($\mathcal{T}_i$, $z_0$)\;
%             % FORWARD EVAL
%             $e_g^i = 0$            \tcp*{graph prediciton error}                                             
%              \For{$\{G_t^i, a^t\}\sim \mathcal{D}_i$}    
%                 { 
%                 	$\hat{G}_i^{j} = $ forward$(G_t^i, a^t, z_i)$\;
%                 	 $e_g^i +=  \lVert \hat{G}_i^{t+1} - G_i^{t+1} \rVert$\;
%                 }
%             % ACTION EVAL
%             $e_a^i = 0$            \tcp*{action prediciton error}                                             
%              \For{$a^j, Goal_j \sim Goals$}    
%                 {   
%                     $G_t^i \sim \mathcal{D}_i$\;
%                 	$a^* =$ getAction$(Goal_j, G_t^i, z_i)$\;
%                 	 $e_a^i += \lVert a^* - a^j \rVert$\;
%                 }
            
%         }
  
  
%   }
%   \;
  

% \label{alg:action}
% \caption{Adaptation evaluation}

% %\end{multicols}
% \end{algorithm}

